One Prompt is not Enough: Automated Construction of a Mixture-of-Expert Prompts

Large Language Models (LLMs) exhibit strong generalization capabilities to novel tasks when prompted with language instructions and in-context demos. Since this ability sensitively depends on the quality of prompts, various methods have been explored to automate the instruction design. While these methods demonstrated promising results, they also restricted the searched prompt to one instruction. Such simplification significantly limits their capacity, as a single demo-free instruction might not be able to cover the entire complex problem space of the targeted task. To alleviate this issue, we adopt the Mixture-of-Expert paradigm and divide the problem space into a set of sub-regions; Each sub-region is governed by a specialized expert, equipped with both an instruction and a set of demos. A two-phase process is developed to construct the specialized expert for each region: (1) demo assignment: Inspired by the theoretical connection between in-context learning and kernel regression, we group demos into experts based on their semantic similarity; (2) instruction assignment: A region-based joint search of an instruction per expert complements the demos assigned to it, yielding a synergistic effect. The resulting method, codenamed Mixture-of-Prompts (MoP), achieves an average win rate of 81% against prior arts across several major benchmarks.

==> algos/_ex.tex <==
\begin{algorithm}[H]
    \caption{A Single Generation Cycle of GEAM}
\begin{algorithmic}
    \STATE \textbf{Input:} Fragment vocabulary $\mathcal{S}$, termination number of atoms in SAC $n_\text{SAC}$, \\
    \quad\quad\quad trained FGIB, population size of GA $P$, maximum vocabulary size $L$
    \STATE \boxit{green}{9} \textit{$\triangleright$ Fragment assembly}
    \STATE Initialize $\rvs_0=\text{benzene}$
    \FOR{$t=0,1,\ldots$}
        \STATE Sample $\rva_t$ from $p_{\pi_1}$, $p_{\pi_2}$ and $p_{\pi_3}$ in Eq.~(\ref{eq:ac1}-\ref{eq:ac3}) with $\mathcal{S}$
        \STATE Construct $\rvs_{t+1}$ by taking $\rva_t$ on $\rvs_t$
        \IF{no attachment point left in $\rvs_{t+1}$ \OR $n_{t+1} > n_\text{SAC}$}
            \STATE $T \leftarrow t+1$
            \STATE break
        \ENDIF
    \ENDFOR
    \STATE Calculate the property $Y$ of $\rvs_T$
    \STATE Set $r_T \leftarrow Y$
    \STATE Train SAC with Eq.~(\ref{eq:sac})
    \STATE \boxit{yellow}{3} \textit{$\triangleright$ Fragment modification}
    \STATE Initialize a population with the top-$P$ molecules generated so far
    \STATE Select parent molecules from the population
    \STATE Perform crossover and mutation to generate an offspring $\rvo$
    \STATE Calculate the property $Y$ of $\rvo$
    \STATE \boxit{blue}{2} \textit{$\triangleright$ Fragment extraction}
    \STATE Extract fragments $\mathcal{S}'$ from $\rvo$ with FGIB
    \STATE Set $\mathcal{S} \leftarrow$ the top-$L$ fragments in $\mathcal{S}\cup\mathcal{S}'$ in terms of Eq.~(\ref{eq:score})
    \STATE \textbf{Output:} Generated molecules ($\rvs_T$ and $\rvo$), updated vocabulary $\mathcal{S}$
\end{algorithmic}
\label{alg:generation}
\end{algorithm}


==> algos/_ex2.tex <==
% If you are using \LaTeX, please use the ``algorithm'' and ``algorithmic''
% environments to format pseudocode. These require
% the corresponding stylefiles, algorithm.sty and
% algorithmic.sty, which are supplied with this package.

\begin{algorithm}[tb]
   \caption{Bubble Sort}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $x_i$, size $m$
   \REPEAT
   \STATE Initialize $noChange = true$.
   \FOR{$i=1$ {\bfseries to} $m-1$}
   \IF{$x_i > x_{i+1}$}
   \STATE Swap $x_i$ and $x_{i+1}$
   \STATE $noChange = false$
   \ENDIF
   \ENDFOR
   \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}

==> figures_tex/demo_clusters.tex <==
\begin{figure*}[t!]
    \centering

    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/icml/cluster/auto_categorization_annot.png}
        \caption{Auto categorization}
        \label{fig:demo_clusters_auto_cate}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/icml/cluster/auto_categorization_annot.png}
        \caption{Logic2text sentence generation}
        \label{fig:demo_clusters_logic}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/icml/cluster/auto_categorization_annot.png}
        \caption{Mathdataset classification}
        \label{fig:demo_clusters_math_class}
    \end{subfigure}

    \caption{\textbf{Illustration of K-means clustering in the embedding space with t-SNE projection.} The circle, triangle, and star shapes represent training, validation, and test demos, respectively. Validation and test demos are routed to experts based on the clustering of training demos using the routing function in \Cref{eq:routing}.}
    \label{fig:demo_clusters_app}
\end{figure*}




==> figures_tex/different_strength/demo_only.tex <==
\begin{figure}[t]
    \centering
 
    \includegraphics[width=0.7\linewidth]{figures/icml/diff_st/auto_categorization.png}
    \label{fig:diff_str_auto_categorization}
    % \includegraphics[width=0.3\linewidth]{figures/different_strength/demo_only/cause_and_effect_bar_plot.png}
    % \label{fig:diff_str_cause_and_effect}
    % \includegraphics[width=0.3\linewidth]{figures/different_strength/demo_only/taxonomy_animal_bar_plot.png}
    % \label{fig:diff_str_taxonomy_animal}

    \caption{\small \textbf{Different experts have different strength.} 
    % To verify the impact of expert assignment for each test input, we calculate the Hit Ratio by counting the number of correctly guessed experts out of the total number of experts for each test input. 
    Test inputs falling within the Hit Ratio range, except for 0/4 and 4/4, indicate that they are influenced by the specific expert they are assigned to, implying that each region’s demos
    define distinct expertise to match queries within their respective local regions.
    % underscoring the significance of assigning the right expert to each test input, which is demonstrated to have a substantial impact on performance. 
    % We run experiments with four different seeds and provide the mean and standard deviation.
    }
    \label{fig:different_strength_demo_only}
    
\end{figure}


==> figures_tex/different_strength/fixed_inst_1.tex <==
\begin{figure}[t]
	\centering
 
        \includegraphics[width=4.3cm]{figures/different_strength/fixed_inst_1/cause_and_effect_bar_plot.png}
	\label{fig:diff_str_cause_and_effect}
         \includegraphics[width=4.3cm]{figures/different_strength/fixed_inst_1/taxonomy_animal_bar_plot.png}
	\label{fig:diff_str_taxonomy_animal}
 %         \includegraphics[width=4.3cm]{figures/viz_demo_clusters/setence_similarity.pdf}
	% \label{fig:viz_demo_clusters_sentence_similarity}
        \includegraphics[width=4.3cm]{figures/different_strength/fixed_inst_1/auto_categorization_bar_plot.png}
	\label{fig:diff_str_auto_categorization}

	\caption{\small \textbf{Different experts have different strength. \sh{(use fixed instruction; cause increased variance?; can we say the result also demonstrate the necessity of joint search for instruction and demos?)}} \sh{figures will be updated...} To verify the impact of expert assignment for each test input, we calculate the Hit Ratio by counting the number of correctly guessed experts out of the total number of experts for each test input. Test inputs falling within the Hit Ratio range, other than 0 and 1, indicate that they are influenced by which expert they are assigned to. In other words, not all experts exert an equal level of influence on each test input, underscoring the significance of assigning the right expert to each test input, which is demonstrated to have a substantial impact on performance.\wrc{add a "win rate"}}
	\label{fig:different_strength_demo_only}
    
\end{figure}


==> figures_tex/main/na_20_2.tex <==
\begin{figure}[t]
	\centering
        
        \includegraphics[width=1.0\textwidth]{figures/main/na_20_2.png}
	\label{fig:main_exp}
	\caption{\small \textbf{Test Accuracy on Instruction Induction tasks within the APE benchmark.} \sh{[Make table for all selected tasks (except too easy task...)?] [Add mop\_random or not?] figures will be updated...} The number of agents is set to 20. We run
experiments with four different random seeds.}
	\label{fig:different_strength_demo_only}
    
\end{figure}


==> figures_tex/main/na_5_2.tex <==
\begin{figure}[t]
	\centering
        
        \includegraphics[width=1.0\textwidth]{figures/main/na_5_2.png}
	\label{fig:main_exp}
	\caption{\small \textbf{Test Accuracy on Instruction Induction tasks within the APE benchmark.} \sh{[Make table for all selected tasks (except too easy task...)?] [Add more tasks] [Add mop\_random or not?] figures will be updated...} The number of agents is set to 5. We run
experiments with four different random seeds.}
	\label{fig:different_strength_demo_only}
    \wrc{I think it might be better to show 5.1 as a line curve (similar to Figure 4) but the x-axis is the number of demos, on 2-3 tasks.}
    
\end{figure}


==> figures_tex/mop_ex.tex <==
\begin{figure*}[ht]
\vskip 0.2in
\centering
\includegraphics[width=1\linewidth]{figures/mop_2.png}
\caption{\small \textbf{The prompts for each expert found by MoP in the \texttt{sentence\_similarity} task.} We provide examples of (instruction, demos) for each expert found by MoP for the \texttt{sentence\_similarity} task. To see the complete results and results for other tasks, please refer to \Cref{appendix:final_prompts_ex}.}
\label{fig:mop_ex}
\vspace{-2mm}
\end{figure*}


==> figures_tex/ranking_change_by_inst/ranking_change_by_inst.tex <==
\begin{figure}[t]
	\centering
 
    \includegraphics[width=0.7\linewidth]{figures/icml/rank/auto_categorization.png}
    \label{fig:diff_rank_auto_categorization}
    % \includegraphics[width=0.3\linewidth]{figures/ranking_change_by_inst/cause_and_effect_rank_plot.png}
    % \label{fig:diff_rank_cause_and_effect}
    % \includegraphics[width=0.3\linewidth]{figures/ranking_change_by_inst/taxonomy_animal_rank_plot.png}
    % \label{fig:diff_rank_taxonomy_animal}
    
    \caption{\small \textbf{Variations in Agent Rankings Across Different Instructions.} The results show the changing rankings among agents when different types of fixed instructions are provided to fixed agents. 
    % We formed four agents using the K-Means clustering algorithm, each using a fixed instruction along with the demo dataset assigned to that agent. 
    As depicted above, varying the fixed instructions results in fluctuations in the agent rankings, and there is no consistently high-performing agent.
    } 
    \label{fig:ranking_change_by_inst}
    
\end{figure}


==> figures_tex/viz_demo_clusters/kmean.tex <==
\begin{figure}[t]
	\centering
 
    \includegraphics[width=0.6\linewidth]{figures/viz_demo_clusters/auto_categorization.png}
    \label{fig:viz_demo_clusters_auto_categorization}
    % \includegraphics[width=0.3\linewidth]{figures/viz_demo_clusters/negation.png}
    % \label{fig:viz_demo_clusters_negation}
    % \includegraphics[width=0.3\linewidth]{figures/viz_demo_clusters/translation_en-es.png}
    % \label{fig:viz_demo_clusters_translate_en-es}

	\caption{\small \textbf{Visualization results of demo clusters.} The results show the clustered demos after being mapped to the embedding space using a text encoder. 
 % We apply the K-Means-Auto clustering algorithm and linearly transform data points in the embedding space using PCA for 2D visualization. 
 Demos belonging to the same cluster are represented with the same color, and example texts within each cluster are shown accordingly. 
 % The visualization results indicate that demo samples with similar semantic meanings tend to cluster closely.
 }
 \label{fig:viz_demo_clusters}
\end{figure}


==> tables/bbh/task_sel_criteria.tex <==
\begin{table*}[h!]
\tiny
    \caption{\small \sh{TODO} \textbf{...}}
    \begin{center}
        
    \resizebox{0.7\linewidth}{!}{
        \begin{tabular}{lll}
            \toprule
            \multicolumn{1}{l}{\multirow{2}{*}{Task}} & \multicolumn{2}{c}{Execution Accuracy (\%)} \\
                                                      & \multicolumn{1}{c}{APE~\citep{zhou2022large}} & \multicolumn{1}{c}{APE + Demos} \\
            
            \midrule
            \midrule

            causal\_judgement                         & 58.87\tiny$\pm$0.50          & 59.57\tiny$\pm$0.87          \\
            disambiguation\_qa                        & 60.00\tiny$\pm$6.48          & 69.33\tiny$\pm$1.25          \\
            dyck\_languages                           & 2.67\tiny$\pm$3.77           & 11.33\tiny$\pm$0.94          \\
            movie\_recommendation                     & 68.67\tiny$\pm$3.30          & 78.67\tiny$\pm$3.30          \\
            navigate                                  & 63.33\tiny$\pm$5.79          & 54.33\tiny$\pm$5.31          \\
            object\_counting                          & 52.33\tiny$\pm$1.89          & 52.00\tiny$\pm$2.94          \\
            ruin\_names                               & 79.67\tiny$\pm$3.30          & 69.67\tiny$\pm$2.62          \\
            snarks                                    & 61.05\tiny$\pm$6.95          & 55.06\tiny$\pm$4.20          \\
            sports\_understanding                     & 75.00\tiny$\pm$10.61         & 87.33\tiny$\pm$0.94          \\
            word\_sorting                             & 67.67\tiny$\pm$0.47          & 78.00\tiny$\pm$0.82          \\
            
            \bottomrule
            \end{tabular}
        }

    \end{center}
    \label{tbl:bbh_task_sel_criteria}
\end{table*}


==> tables/ex_sentence_similarity.tex <==
% \setstcolor{red}
\begin{table}[t!]
\tiny
\centering
\caption{\small \textbf{The prompts for each expert found by MoP in the \texttt{sentence\_similarity} task.} We provide examples of (instruction, demos) for each expert found by MoP for the \texttt{sentence\_similarity} task. To see the complete results and results for other tasks, please refer to \Cref{appendix:final_prompts_ex}.}
\resizebox{1.00\textwidth}{!}{
    \renewcommand{\arraystretch}{0.95}
    \begin{tabular}{ll}
    \toprule
    % \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task}: sentence\_similarity} \\
    % \midrule
    {} & \multicolumn{1}{c}{\textbf{Prompts}} \\
    \midrule
    \midrule
    \multirowcell{2}[-0.0ex][l]{Expert \\ 1/6}
    & \multicolumn{1}{p{0.9\textwidth}}{\textcolor{blue}{\textbf{Instruction}}: create two sentences that convey similar information, but the second sentence should have a different wording or phrasing compared to the first sentence. The output indicates the level of similarity between the two sentences, with 5 being a perfect match and 1 being highly. \newline
    \textcolor{magenta}{\textbf{Demos}}: Input: \textbf{Sentence 1}: Two people sit on the end of a dock. Sentence 2: Two people sitting on a dock.$\backslash$nOutput: 4 - almost perfectly$\backslash$n$\backslash$nInput: \textbf{Sentence 1}: Two people sit on the end of a dock. Sentence 2: Two people sitting on a dock.$\backslash$nOutput: 4 - almost perfectly$\backslash$n$\backslash$nInput: \textbf{Sentence 1}: Two people sit on the end of a dock. Sentence 2: Two people sitting on a dock.$\backslash$nOutput: 4 - almost perfectly, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
   \multirowcell{2}[-0.0ex][l]{Expert \\ 2/6}
    & \multicolumn{1}{p{0.9\textwidth}}{\textcolor{blue}{\textbf{Instruction}}: determine the similarity of two sentences. The output numbers represent the level of similarity, with 1 being the lowest and 5 being the highest. \newline
    \textcolor{magenta}{\textbf{Demos}}: Input: \textbf{Sentence 1}: A dog swimming with a stick in it's mouth. Sentence 2: A dog running with a stick in it's mouth.$\backslash$nOutput: 3 - probably$\backslash$n$\backslash$nInput: \textbf{Sentence 1}: A dog is running on the ground. Sentence 2: A girl is tapping her finger nails.$\backslash$nOutput: 0 - definitely not, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    % $\vdots$
    \multirowcell{1}[-0.0ex][l]{}
    & \multicolumn{1}{c}{$\vdots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 6/6}
    & \multicolumn{1}{p{0.9\textwidth}}{\textcolor{blue}{\textbf{Instruction}}: create two sentences that convey similar information, but the second sentence should have a different wording or phrasing compared to the first sentence. The output indicates the level of similarity between the two sentences, with 5 being a perfect match and 1 being highly. \newline
    \textcolor{magenta}{\textbf{Demos}}: Input: \textbf{Sentence 1}: Israel's Peres urges return to peace talks Sentence 2: Gonsalves keeps up pressure on Dom Rep$\backslash$nOutput: 0 - definitely not$\backslash$n$\backslash$nInput: \textbf{Sentence 1}: Israeli, Palestinian negotiators quietly meet Sentence 2: Israeli, Palestinian negotiators meet in Jordan$\backslash$nOutput: 4 - almost perfectly, $\ldots$} \\
    % \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}

    \bottomrule
    \end{tabular}
}
\label{tab:ex_sentence_sim}
\vspace{-0.175in}
\end{table}


==> tables/final_prompts.tex <==
\begin{table*}[t!]
    \caption{\small \textbf{The best prompts proposed by MoP + K-Means-Auto} ...}
    \begin{center}
        
    \resizebox{\linewidth}{!}{
        \begin{tabular}{lcc}
            \toprule
            
            \multicolumn{1}{l}{\multirow{1}{*}{Task}} & 
            \multicolumn{1}{c}{Expert ID} & 
            \multicolumn{1}{c}{Prompts} \\
            
            \midrule
            \midrule

            \multicolumn{1}{c}{\multirow{8}{*}{auto\_categorization}} & 
            1  & 
            Instruction:  group or categorize the items into related or similar groups. The input-output pairs all demonstrate this by organizing the items into categories such as journals, apparel, people shot by police, historical wars, presidents of the U.S, animals, computer science books$\backslash$ n $\backslash$ n Input:  John Adams, Millard Fillmore, and Grover Cleveland   $\backslash$ n Output: presidents of the U.S$\backslash$ n $\backslash$ n Input: Benin, Zambia, and Mauritius $\backslash$ n Output: African countries$\backslash$ n $\backslash$ n Input: Nigeria, Russia, and Egypt$\backslash$ n Output: countries with large population$\backslash$ n $\backslash$ n Input: Philippines, Brazil, and India  $\backslash$ n Output: countries with large population$\backslash$ n $\backslash$ n Input:  Togo, Eritrea, and Burundi   $\backslash$ n Output: African countries$\backslash$ n $\backslash$ n Input: AUSTRO-ITALIAN WAR, JACOBITE REBELLION, and FRANCO-SPANISH WAR$\backslash$ n Output: historical wars$\backslash$ n $\backslash$ n Input:  Botswana, Cameroon, and Ivory Coast   $\backslash$ n Output: African countries$\backslash$ n $\backslash$ n Input: Europe, Australia, and South America $\backslash$ n Output: continents \\
            &
            2 & 
            Instruction:  group or categorize the items into related or similar groups. The input-output pairs all demonstrate this by organizing the items into categories such as journals, apparel, people shot by police, historical wars, presidents of the U.S, animals, computer science books$\backslash$ n $\backslash$ n Input: Sports Shoes, Shorts, and Sweaters$\backslash$ n Output: Apparel$\backslash$ n $\backslash$ n Input: water, ethanol, acetone, and methanol$\backslash$ n Output: solvant$\backslash$ n $\backslash$ n Input:  Charizard, Lugia, and Piplup   $\backslash$ n Output: pokeman$\backslash$ n $\backslash$ n Input:   Sailing, Fencing, and Roque $\backslash$ n Output: sports$\backslash$ n $\backslash$ n Input: wsstyles, json, and ws $\backslash$ n Output: computer file format extensions$\backslash$ n $\backslash$ n Input: Drifblim, Squirtle, and Rayquaza$\backslash$ n Output: pokeman$\backslash$ n $\backslash$ n Input:   DemandBase, InfusionSoft, and HotSchedules $\backslash$ n Output: tech companies$\backslash$ n $\backslash$ n Input: Jeans, Tops, and Suits$\backslash$ n Output: Apparel \\
            &
            3 & 
            Instruction:  group similar items together based on a common characteristic or category. The output for each input is the category or characteristic that the items share.$\backslash$ n $\backslash$ n Input:  Sharanahua, Chairel, and Tafi$\backslash$ n Output: extinct languages$\backslash$ n $\backslash$ n Input: Building of meteorological station, Manor Kozhin, and Watch tower$\backslash$ n Output: tourist_attractions$\backslash$ n $\backslash$ n Input:   Con Calma, 7 rings, and Truth Hurts $\backslash$ n Output: popular songs$\backslash$ n $\backslash$ n Input: Sheera, Bajri no rotlo, and Unni Appam  $\backslash$ n Output: indian foods$\backslash$ n $\backslash$ n Input: The building of the gymnasium, Historical Reserve - the ruins of the mill them. KN Grudinina, and Chamber Stroganoff$\backslash$ n Output: tourist_attractions$\backslash$ n $\backslash$ n Input:   Ngardi, Klallam, and Old Prussian $\backslash$ n Output: extinct languages$\backslash$ n $\backslash$ n Input: Vera'a, Maniwaki Algonquin, and Swoeng$\backslash$ n Output: extinct languages$\backslash$ n $\backslash$ n Input: Khichu, Chapati, and Sev khamani $\backslash$ n Output: indian foods \\
            &
            4 &
            Instruction: $\backslash$ n $\backslash$ n Input:  Kotlin, Java, and Matlab$\backslash$ n Output: programming languages$\backslash$ n $\backslash$ n Input: Python, Cobol, and C#$\backslash$ n Output: programming languages$\backslash$ n $\backslash$ n Input: A History, a Theory, a Flood, How Google Works, and The Code Book: The Science of Secrecy from Ancient Egypt to Quantum Cryptography$\backslash$ n Output: Computer Science books$\backslash$ n $\backslash$ n Input: Stirling's approximation, Shannon\u2013Hartley theorem, and Schottky's theorem $\backslash$ n Output: math theorems$\backslash$ n $\backslash$ n Input: The Architecture of Open Source Applications, Algorithms to Live By: The Computer Science of Human Decisions, and The Art of the Start: The Time-Tested, Battle-Hardened Guide for Anyone Starting Anything  $\backslash$ n Output: Computer Science books$\backslash$ n $\backslash$ n Input: ICGA, IEEE, and Journal of the ACM$\backslash$ n Output: Computer Science journals$\backslash$ n $\backslash$ n Input: Computer Coding, Sync: The Emerging Science of Spontaneous Order, and The Hidden Connections: A Science for Sustainable Living $\backslash$ n Output: Computer Science books$\backslash$ n $\backslash$ n Input: Liouville's theorem, Pu's inequality, and Picard$\backslash$ u2013Lindel$\backslash$ u00f6f theorem  $\backslash$ n Output: math theorems \\
            &
            5 &
            Instruction: $\backslash$ n $\backslash$ n Input:   Mikhail Vrubel, Rene Magritte, and Amedeo Modigliani  $\backslash$ n Output: artists$\backslash$ n $\backslash$ n Input:   James Bauduy, Patrick Bryant, and Elman Jerald Roberts $\backslash$ n Output: people shot by police$\backslash$ n $\backslash$ n Input: Marie Curie, Albert Einstein, Mo Yan, Michael Houghton have all won$\backslash$ n Output: the Nobel Prize$\backslash$ n $\backslash$ n Input: Tameka LaShay Simpson, Leslie Sapp III, and Edward Manning  $\backslash$ n Output: people shot by police$\backslash$ n $\backslash$ n Input: Augusta Savage, Louise Bourgeois, Mary Cassatt, and Elaine Sturtevant$\backslash$ n Output: female artist$\backslash$ n $\backslash$ n Input:   Mikhail Vrubel, Rene Magritte, and Amedeo Modigliani  $\backslash$ n Output: artists$\backslash$ n $\backslash$ n Input:   James Bauduy, Patrick Bryant, and Elman Jerald Roberts $\backslash$ n Output: people shot by police$\backslash$ n $\backslash$ n Input: Marie Curie, Albert Einstein, Mo Yan, Michael Houghton have all won$\backslash$ n Output: the Nobel Prize \\
            &
            6 &
            Instruction: $\backslash$ n $\backslash$ n Input: TeenVogue.com, NME, and Tampa Bay Review$\backslash$ n Output: the media$\backslash$ n $\backslash$ n Input:  Physics Reports, Advanced Materials, and The Lancet Oncology $\backslash$ n Output: top journals$\backslash$ n $\backslash$ n Input: Government of Ontario News, WMTV, and La Crosse Tribune $\backslash$ n Output: the media$\backslash$ n $\backslash$ n Input: WhoWhatWhy / RealNewsProject (blog), Today.com, and Rockford Register Star$\backslash$ n Output: the media$\backslash$ n $\backslash$ n Input: TeenVogue.com, NME, and Tampa Bay Review$\backslash$ n Output: the media$\backslash$ n $\backslash$ n Input:  Physics Reports, Advanced Materials, and The Lancet Oncology $\backslash$ n Output: top journals$\backslash$ n $\backslash$ n Input: Government of Ontario News, WMTV, and La Crosse Tribune $\backslash$ n Output: the media$\backslash$ n $\backslash$ n Input: WhoWhatWhy / RealNewsProject (blog), Today.com, and Rockford Register Star$\backslash$ n Output: the media \\
            &
            7 &
            Instruction:  list things that fall into a certain category or theme.$\backslash$ n $\backslash$ n Input: Azuchi-Momoyama period, Edo period, and Reiwa period $\backslash$ n Output: periods of Japanese history$\backslash$ n $\backslash$ n Input: EverQuest II, Ikaruga, and State of Decay  $\backslash$ n Output: games on Steam$\backslash$ n $\backslash$ n Input: Wildlife Park 2 - Crazy Zoo, Glorkian Warrior The Trials Of Glork, and Software Inc. $\backslash$ n Output: games on Steam$\backslash$ n $\backslash$ n Input: Azuchi-Momoyama period, Edo period, and Reiwa period $\backslash$ n Output: periods of Japanese history$\backslash$ n $\backslash$ n Input: EverQuest II, Ikaruga, and State of Decay  $\backslash$ n Output: games on Steam$\backslash$ n $\backslash$ n Input: Wildlife Park 2 - Crazy Zoo, Glorkian Warrior The Trials Of Glork, and Software Inc. $\backslash$ n Output: games on Steam$\backslash$ n $\backslash$ n Input: Azuchi-Momoyama period, Edo period, and Reiwa period $\backslash$ n Output: periods of Japanese history$\backslash$ n $\backslash$ n Input: EverQuest II, Ikaruga, and State of Decay  $\backslash$ n Output: games on Steam \\
            &
            8 &
            Instruction:  group or categorize the items into related or similar groups. The input-output pairs all demonstrate this by organizing the items into categories such as journals, apparel, people shot by police, historical wars, presidents of the U.S, animals, computer science books$\backslash$ n $\backslash$ n Input: Nature Nanotechnology, Annual Review of Biochemistry, and The Lancet Neurology $\backslash$ n Output: top journals$\backslash$ n $\backslash$ n Input: Rubella, Tetanus, and Varicella Hospitalizations$\backslash$ n Output: vaccine preventable diseases$\backslash$ n $\backslash$ n Input:  Plague, human, Dengue Virus Infection, and Cryptosporidiosis $\backslash$ n Output: infectious diseases$\backslash$ n $\backslash$ n Input: Cysticercosis or Taeniasis, Anthrax, and Listeriosis $\backslash$ n Output: infectious diseases$\backslash$ n $\backslash$ n Input: Ribosomes, plasmid, cell wall, and plasma membrane$\backslash$ n Output: prokaryotic cells$\backslash$ n $\backslash$ n Input:  E. coli O157, Cyclosporiasis, and Relapsing Fever   $\backslash$ n Output: infectious diseases$\backslash$ n $\backslash$ n Input: Botulism, Foodborne, Campylobacteriosis, and Lyme Disease$\backslash$ n Output: infectious diseases$\backslash$ n $\backslash$ n Input: Hurricanes, floods, and earthquakes$\backslash$ n Output: natural disasters \\
            
            \bottomrule
            
            \end{tabular}
        }
    \end{center}
    \label{tbl:final_prompts_ex}
\end{table*}

==> tables/final_prompts_ex/auto_categorization.tex <==
% \setstcolor{red}
\begin{table}[t!]
\footnotesize
\centering
\caption{\small \textbf{The prompts for each expert found by MoP in the auto\_categorization task of the APE benchmark~\citep{honovich2022instruction}.}}
\resizebox{1.00\textwidth}{!}{
    \renewcommand{\arraystretch}{0.95}
    \begin{tabular}{ll}
    \toprule
    % \multicolumn{3}{p{1.3\textwidth}}{\textbf{Instruction}: The following are multiple-choice questions about medical knowledge. Generate step-by-step explanations for each question.} \\
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task}: auto\_categorization} \\
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task Summary}: Categorize items based on a common theme or characteristic.} \\
    \midrule
    {} & \multicolumn{1}{c}{\textbf{Prompts}} \\
    % {} & \multicolumn{1}{c}{\textbf{Retrieved Passage}} & \multicolumn{1}{c}{\textbf{Prompts}} \\
    \midrule
    \midrule
    \multirowcell{2}[-0.0ex][l]{Expert \\ 1/8}
    % \multirowcell{2}[-0.0ex][l]{\textbf{Expert 1/8} \\ \textit{(Ours, reranker)}}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: group or categorize the items into related or similar groups. The input-output pairs all demonstrate this by organizing the items into categories such as journals, apparel, people shot by police, historical wars, presidents of the U.S, animals, computer science books \newline
    \textbf{Demos}: Input: Benin, Zambia, and Mauritius $\backslash$nOutput: African countries$\backslash$n$\backslash$nInput: Nigeria, Russia, and Egypt$\backslash$nOutput: countries with large population$\backslash$n$\backslash$nInput: Philippines, Brazil, and India  $\backslash$nOutput: countries with large population$\backslash$n$\backslash$nInput:  Togo, Eritrea, and Burundi   $\backslash$nOutput: African countries $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    \multirowcell{2}[-0.0ex][l]{Expert \\ 2/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:  \newline
    \textbf{Demos}: Input: Python, Cobol, and C\#$\backslash$nOutput: programming languages$\backslash$n$\backslash$nInput:  Kotlin, Java, and Matlab$\backslash$nOutput: programming languages$\backslash$n$\backslash$nInput: A History, a Theory, a Flood, How Google Works, and The Code Book: The Science of Secrecy from Ancient Egypt to Quantum Cryptography$\backslash$nOutput: Computer Science books $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    \multirowcell{2}[-0.0ex][l]{Expert \\ 3/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:  group or categorize the items into related or similar groups. The input-output pairs all demonstrate this by organizing the items into categories such as journals, apparel, people shot by police, historical wars, presidents of the U.S, animals, computer science books \newline
    \textbf{Demos}: Input: Sports Shoes, Shorts, and Sweaters$\backslash$nOutput: Apparel$\backslash$n$\backslash$nInput: Jeans, Tops, and Suits$\backslash$nOutput: Apparel, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    \multirowcell{2}[-0.0ex][l]{Expert \\ 4/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:  group similar items together based on a common characteristic or category. The output for each input is the category or characteristic that the items share. \newline
    \textbf{Demos}: Input:  Sharanahua, Chairel, and Tafi$\backslash$nOutput: extinct languages$\backslash$n$\backslash$nInput:   Ngardi, Klallam, and Old Prussian $\backslash$nOutput: extinct languages$\backslash$n$\backslash$nInput: Building of meteorological station, Manor Kozhin, and Watch tower$\backslash$nOutput: tourist\_attractions$\backslash$n$\backslash$nInput: The building of the gymnasium, Historical Reserve - the ruins of the mill them. KN Grudinina, and Chamber Stroganoff$\backslash$nOutput: tourist\_attractions$\backslash$n$\backslash$nInput: Vera'a, Maniwaki Algonquin, and Swoeng$\backslash$nOutput: extinct languages, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    \multirowcell{2}[-0.0ex][l]{Expert \\ 5/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: \newline 
    \textbf{Demos}: Input: Mikhail Vrubel, Rene Magritte, and Amedeo Modigliani  $\backslash$nOutput: artists$\backslash$n$\backslash$nInput:   James Bauduy, Patrick Bryant, and Elman Jerald Roberts $\backslash$nOutput: people shot by police$\backslash$n$\backslash$nInput: Marie Curie, Albert Einstein, Mo Yan, Michael Houghton have all won$\backslash$nOutput: the Nobel Prize$\backslash$n$\backslash$nInput: Tameka LaShay Simpson, Leslie Sapp III, and Edward Manning  $\backslash$nOutput: people shot by police$\backslash$n$\backslash$nInput: Augusta Savage, Louise Bourgeois, Mary Cassatt, and Elaine Sturtevant$\backslash$nOutput: female artist$\backslash$n$\backslash$nInput:   Mikhail Vrubel, Rene Magritte, and Amedeo Modigliani  $\backslash$nOutput: artists$\backslash$n$\backslash$nInput:   James Bauduy, Patrick Bryant, and Elman Jerald Roberts $\backslash$nOutput: people shot by police$\backslash$n$\backslash$nInput: Marie Curie, Albert Einstein, Mo Yan, Michael Houghton have all won$\backslash$nOutput: the Nobel Prize, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    \multirowcell{2}[-0.0ex][l]{Expert \\ 6/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:  list things that fall into a certain category or theme. \newline
    \textbf{Demos}: Input: Azuchi-Momoyama period, Edo period, and Reiwa period $\backslash$nOutput: periods of Japanese history$\backslash$n$\backslash$nInput: EverQuest II, Ikaruga, and State of Decay  $\backslash$nOutput: games on Steam$\backslash$n$\backslash$nInput: Wildlife Park 2 - Crazy Zoo, Glorkian Warrior The Trials Of Glork, and Software Inc. $\backslash$nOutput: games on Steam$\backslash$n$\backslash$nInput: EverQuest II, Ikaruga, and State of Decay  $\backslash$nOutput: games on Steam$\backslash$n$\backslash$nInput: Wildlife Park 2 - Crazy Zoo, Glorkian Warrior The Trials Of Glork, and Software Inc. $\backslash$nOutput: games on Steam, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    \multirowcell{2}[-0.0ex][l]{Expert \\ 7/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:  group or categorize the items into related or similar groups. The input-output pairs all demonstrate this by organizing the items into categories such as journals, apparel, people shot by police, historical wars, presidents of the U.S, animals, computer science books \newline
    \textbf{Demos}: Input: Rubella, Tetanus, and Varicella Hospitalizations$\backslash$nOutput: vaccine preventable diseases$\backslash$n$\backslash$nInput:  Plague, human, Dengue Virus Infection, and Cryptosporidiosis $\backslash$nOutput: infectious diseases$\backslash$n$\backslash$nInput: Cysticercosis or Taeniasis, Anthrax, and Listeriosis $\backslash$nOutput: infectious diseases$\backslash$n$\backslash$nInput: Ribosomes, plasmid, cell wall, and plasma membrane$\backslash$nOutput: prokaryotic cells, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    \multirowcell{2}[-0.0ex][l]{Expert \\ 8/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: \newline
    \textbf{Demos}: Input: TeenVogue.com, NME, and Tampa Bay Review$\backslash$nOutput: the media$\backslash$n$\backslash$nInput: Government of Ontario News, WMTV, and La Crosse Tribune $\backslash$nOutput: the media$\backslash$n$\backslash$nInput: WhoWhatWhy / RealNewsProject (blog), Today.com, and Rockford Register Star$\backslash$nOutput: the media$\backslash$n$\backslash$nInput: TeenVogue.com, NME, and Tampa Bay Review$\backslash$nOutput: the media$\backslash$n$\backslash$nInput:  Physics Reports, Advanced Materials, and The Lancet Oncology $\backslash$nOutput: top journals, $\ldots$} \\

    \bottomrule
    \end{tabular}
}
\label{tab:appendix_ex_auto_cate}
% \vspace{-0.175in}
\end{table}

==> tables/final_prompts_ex/negation.tex <==
% \setstcolor{red}
\begin{table}[t!]
\footnotesize
\centering
\caption{\small \textbf{The prompts for each expert found by MoP in the negation task of the APE benchmark~\citep{honovich2022instruction}.}}
\resizebox{1.00\textwidth}{!}{
    \renewcommand{\arraystretch}{0.95}
    \begin{tabular}{ll}
    \toprule
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task}: negation} \\
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task Summary}: Negate the input sentence.} \\
    \midrule
    {} & \multicolumn{1}{c}{\textbf{Prompts}} \\
    \midrule
    \midrule
    \multirowcell{2}[-0.0ex][l]{Expert \\ 1/3}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: negate the verb or verb phrase in the input sentence. \newline
    \textbf{Demos}: Input: Crawfordsburn is a village.$\backslash$nOutput: Crawfordsburn is not a village.$\backslash$n$\backslash$nInput: Victoria's largest non-Christian religion is Buddhism.$\backslash$nOutput: Victoria's largest non-Christian religion is not Buddhism. $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 2/3}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: take a statement and negate it. \newline
    \textbf{Demos}: Input: Des Abbott was born in Darwin.$\backslash$nOutput: Des Abbott was not born in Darwin.$\backslash$n$\backslash$nInput: Ellie Tesher was born in Toronto.$\backslash$nOutput: Ellie Tesher was not born in Toronto.$\backslash$n$\backslash$nInput: Paul Daniels was born in Burlington.$\backslash$nOutput: Paul Daniels was not born in Burlington. $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 3/3}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:  negate the verb or verb phrase in the input sentence. \newline
    \textbf{Demos}: Input: Trains can brake.$\backslash$nOutput: Trains cannot brake.$\backslash$n$\backslash$nInput: Casper is a ghost.$\backslash$nOutput: Casper is not a ghost.$\backslash$n$\backslash$nInput: Chlorine can be poisonous.$\backslash$nOutput: Chlorine cannot be poisonous. $\ldots$} \\
    % \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}

    \bottomrule
    \end{tabular}
}
\label{tab:appendix_ex_negation}
% \vspace{-0.175in}
\end{table}


==> tables/final_prompts_ex/orthography_starts_with.tex <==
% \setstcolor{red}
\begin{table}[t!]
\footnotesize
\centering
\caption{\small \textbf{The prompts for each expert found by MoP in the orthography\_starts\_with task of the APE benchmark~\citep{honovich2022instruction}.}}
\resizebox{1.00\textwidth}{!}{
    \renewcommand{\arraystretch}{0.95}
    \begin{tabular}{ll}
    \toprule
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task}: orthography\_starts\_with} \\
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task Summary}: Extract the words starting with a given letter from the input sentence.} \\
    \midrule
    {} & \multicolumn{1}{c}{\textbf{Prompts}} \\
    \midrule
    \midrule
    \multirowcell{2}[-0.0ex][l]{Expert \\ 1/3}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: identify the word that comes after the specified letter in each input sentence. \newline
    \textbf{Demos}: Input: Michael accidentally broke the glass. [m]$\backslash$nOutput: michael$\backslash$n$\backslash$nInput: It was the man that bought the articles from him. [w]$\backslash$nOutput: was$\backslash$n$\backslash$nInput: The fans were deliberately provoked by a rival group. [p]$\backslash$nOutput: provoked$\backslash$n$\backslash$nInput: What Henri wants is the book which is on the top shelf. [s]$\backslash$nOutput: shelf$\backslash$n$\backslash$nInput: This theorem will take only five minutes to prove. [m]$\backslash$nOutput: minutes,  $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 2/3}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: identify the word that comes directly after the designated letter in the input sentence. So for example, for input [a], the output is "about" because it comes directly after the letter "a" in the sentence "John talked to Bill about the \newline
    \textbf{Demos}: Input: These are the things for which to be thankful. [a]$\backslash$nOutput: are$\backslash$n$\backslash$nInput: Water filled the cup. [c]$\backslash$nOutput: cup$\backslash$n$\backslash$nInput: for discussion of the same phenomenon in Russian. [r]$\backslash$nOutput: russian$\backslash$n$\backslash$nInput: I know several people who she kissed. [i]$\backslash$nOutput: i$\backslash$n$\backslash$nInput: I ate fruit [a]$\backslash$nOutput: ate$\backslash$n$\backslash$nInput: We like our friends and they like their friends, too. [a]$\backslash$nOutput: and$\backslash$n$\backslash$nInput: I know several people who she kissed. [s]$\backslash$nOutput: several she, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 3/3}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:  identify the word that comes after the specified letter in each input sentence. \newline
    \textbf{Demos}: Input: Being honest is not an easy task. [i]$\backslash$nOutput: is$\backslash$n$\backslash$nInput: Almost any lawyer could answer that question. [t]$\backslash$nOutput: that$\backslash$n$\backslash$nInput: They denied the claim that they should report only to us. [c]$\backslash$nOutput: claim$\backslash$n$\backslash$nInput: John talked to Bill about the exam. [a]$\backslash$nOutput: about$\backslash$n$\backslash$nInput: We expect the dentist to examine us. [d]$\backslash$nOutput: dentist$\backslash$n$\backslash$nInput: He made a statement which everyone thought was really interesting and important. [t]$\backslash$nOutput: thought$\backslash$n$\backslash$nInput: I wonder what John bought. [w]$\backslash$nOutput: wonder what$\backslash$n$\backslash$nInput: June covered the baby with a blanket. [j]$\backslash$nOutput: june$\backslash$n$\backslash$nInput: We persuaded the dentist to examine us. [w]$\backslash$nOutput: we$\backslash$n$\backslash$nInput: So eminent a scholar as Dr. Lucille Hein was here. [e], $\ldots$} \\
    % \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}

    \bottomrule
    \end{tabular}
}
\label{tab:appendix_ex_orth}
% \vspace{-0.175in}
\end{table}


==> tables/final_prompts_ex/sentence_similarity.tex <==
% \setstcolor{red}
\begin{table}[h]
\footnotesize
\centering
\caption{\small \textbf{The prompts for each expert found by MoP in the sentence\_similarity task.}}
\resizebox{1.00\textwidth}{!}{
    \renewcommand{\arraystretch}{0.95}
    \begin{tabular}{ll}
    \toprule
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task}: sentence\_similarity} \\
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task Summary}: Rate the semantic similarity of two input sentences on a scale of 0 - definitely not to 5 - perfectly.} \\
    \midrule
    {} & \multicolumn{1}{c}{\textbf{Prompts}} \\
    \midrule
    \midrule
    \multirowcell{2}[-0.0ex][l]{Expert \\ 1/6}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: create two sentences that convey similar information, but the second sentence should have a different wording or phrasing compared to the first sentence. The output indicates the level of similarity between the two sentences, with 5 being a perfect match and 1 being highly. \newline
    \textbf{Demos}: Input: Sentence 1: Two people sit on the end of a dock. Sentence 2: Two people sitting on a dock.$\backslash$nOutput: 4 - almost perfectly$\backslash$n$\backslash$nInput: Sentence 1: Two people sit on the end of a dock. Sentence 2: Two people sitting on a dock.$\backslash$nOutput: 4 - almost perfectly$\backslash$n$\backslash$nInput: Sentence 1: Two people sit on the end of a dock. Sentence 2: Two people sitting on a dock.$\backslash$nOutput: 4 - almost perfectly, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 2/6}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: create two sentences that convey similar information, but the second sentence should have a different wording or phrasing compared to the first sentence. The output indicates the level of similarity between the two sentences, with 5 being a perfect match and 1 being highly. \newline
    \textbf{Demos}: Input: Sentence 1: Israel's Peres urges return to peace talks Sentence 2: Gonsalves keeps up pressure on Dom Rep$\backslash$nOutput: 0 - definitely not$\backslash$n$\backslash$nInput: Sentence 1: Israeli, Palestinian negotiators quietly meet Sentence 2: Israeli, Palestinian negotiators meet in Jordan$\backslash$nOutput: 4 - almost perfectly, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 3/6}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: compare the two sentences and determine how similar they are, giving a rating of 1 to 5 (with 1 being not similar at all and 5 being very similar). \newline
    \textbf{Demos}: Input: Sentence 1: Four men admit London Stock Exchange bomb plot Sentence 2: Four men admit London bombs plot$\backslash$nOutput: 4 - almost perfectly$\backslash$n$\backslash$nInput: Sentence 1: Five men in tuxedos are walking down steps. Sentence 2: Five men in tuxedos walk down a set of steps$\backslash$nOutput: 5 - perfectly, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}

    \multirowcell{2}[-0.0ex][l]{Expert \\ 4/6}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: determine the similarity of two sentences. The output numbers represent the level of similarity, with 1 being the lowest and 5 being the highest. \newline
    \textbf{Demos}: Input: Sentence 1: A man is playing the trumpet. Sentence 2: Someone is playing with a toad.$\backslash$nOutput: 1 - probably not$\backslash$n$\backslash$nInput: Sentence 1: A man is slicing a potato. Sentence 2: A woman is cutting a jalepeno.$\backslash$nOutput: 1 - probably not, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}

    \multirowcell{2}[-0.0ex][l]{Expert \\ 5/6}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: \newline
    \textbf{Demos}: Input: Sentence 1: U.S. Drone Kills Five Militants in Pakistan Sentence 2: Six Police Officers Killed in Attacks in Dagestan$\backslash$nOutput: 0 - definitely not$\backslash$n$\backslash$nInput: Sentence 1: P.G. police seeking driver in crash that killed child Sentence 2: Police seek gunmen in New Orleans Mother's Day parade shooting$\backslash$nOutput: 0 - definitely not, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}

    \multirowcell{2}[-0.0ex][l]{Expert \\ 6/6}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: determine the similarity of two sentences. The output numbers represent the level of similarity, with 1 being the lowest and 5 being the highest. \newline
    \textbf{Demos}: Input: Sentence 1: A dog swimming with a stick in it's mouth. Sentence 2: A dog running with a stick in it's mouth.$\backslash$nOutput: 3 - probably$\backslash$n$\backslash$nInput: Sentence 1: A dog is running on the ground. Sentence 2: A girl is tapping her finger nails.$\backslash$nOutput: 0 - definitely not, $\ldots$} \\
    % \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}

    \bottomrule
    \end{tabular}
}
\label{tab:appendix_ex_sentence_sim}
\vspace{-0.175in}
\end{table}


==> tables/rebuttal/comp_w_ensemble.tex <==

% \begin{table}[t!]
% \caption{\small \textbf{Performance } }
% \vspace{-0.1in}
% \tiny
% \begin{center}
% \resizebox{0.7\textwidth}{!}{
% \begin{tabular}{lccc}
% \toprule
%   & sentence\_similarity    & word\_in\_context  & auto\_categorization  \\
                           
% \midrule
% \midrule
% Route to one expert                                   & \textbf{43.00 \tiny$\pm$ 3.54} & \textbf{59.00 \tiny$\pm$ 5.15} & \textbf{54.25 \tiny$\pm$ 2.49} \\ 
% Ensemble of all experts                                  & 15.25 \tiny$\pm$ 17.71 & 52.75 \tiny$\pm$ 7.76 & 0.75 \tiny$\pm$ 1.30 \\  
% \bottomrule
% \end{tabular}
% } 	
% \end{center}
% \label{tbl:suppl_comp_w_ensemble}
% \vspace{-0.15in}
% \end{table}


==> tables/rebuttal/cot.tex <==
\begin{table*}[h!]
\tiny
    \caption{\rebuttal{\textbf{Results on Chain-of-Thought (CoT) Reasoning benchmark task.} We report the execution accuracy for each method on CoT reasoning tasks. Note that the original CoT paper only provides a limited number of human-crafted demos (8); we instead sample demos directly from the dataset for all methods. We run 4 experiments and provide both the mean and standard deviation values. Due to innate randomness in ChatGPT API, we mark methods to be equivalent when their accuracy gap falls within 1\%. The number of demos is set to $N_{\text{train}}/10$, where $N_{\text{train}}$ is the total number of training demos.}}
    \begin{center}
        
    \resizebox{0.5\linewidth}{!}{
        \begin{tabular}{lcccc}
            \toprule
            \multicolumn{1}{l}{\multirow{2}{*}{Task}}      & \multicolumn{4}{c}{Execution Accuracy (\%)} \\
                                                           & APE~\citep{zhou2022large}    & APE+Demos & MoP \\
            
            \midrule
            \midrule

            GSM8K                         & 44.50\tiny$\pm$5.12          & 70.50\tiny$\pm$2.18    & \textbf{74.25\tiny$\pm$0.83}              \\
            MultiArith                    & 82.25\tiny$\pm$13.55          & \textbf{97.00\tiny$\pm$0.00}     & \textbf{97.50\tiny$\pm$2.29}              \\

            \bottomrule
            
            \end{tabular}
        }
    \end{center}
    \label{tbl:cot}
\end{table*}

==> tables/rebuttal/fianl_prompts/superni/dbg.tex <==
% \setstcolor{red}
\begin{table}[t!]
\footnotesize
\centering
\caption{\small \textbf{The prompts for each expert found by MoP in the code\_x\_glue\_information\_retreival task.}}
\resizebox{1.00\textwidth}{!}{
    \renewcommand{\arraystretch}{0.95}
    \begin{tabular}{ll}
    \toprule
    
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task}: code\_x\_glue\_information\_retreival} \\
    \midrule
    {} & \multicolumn{1}{c}{\textbf{Prompts}} \\
    
    \midrule
    \midrule

    % \multirowcell{2}[-0.0ex][l]{Expert \\ 0/8}
    % & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: create a function that counts the number of prime factors of a given number. The input-output pairs show different implementations of this function, with different variable names and control structures. The output values represent the number of prime factors for the given input number. \newline
    % \textbf{Demos}: Input: void f(int i,int m);\textbackslash{}nint sum;\textbackslash{}nint main()\textbackslash{}n\{\textbackslash{}n int n,i,m,k;\textbackslash{}n scanf(\textbackslash{}"\%d\textbackslash{}",\&n);\textbackslash{}n for(i=0;i\textless{}n;i++)\textbackslash{}n \{ sum=1;\textbackslash{}n scanf(\textbackslash{}"\%d\textbackslash{}",\&m);\textbackslash{}n f(2,m);\textbackslash{}n printf(\textbackslash{}"\%d\textbackslash{}\textbackslash{}n\textbackslash{}",sum);\textbackslash{}n \textbackslash{}n \}\textbackslash{}n\}\textbackslash{}n void f(int i ,int m)\textbackslash{}n \{\textbackslash{}n int k,s;\textbackslash{}n s=(int)sqrt(m);\textbackslash{}n for(k=i;k\textless{}=s;k++)\textbackslash{}n \{\textbackslash{}n if(m\%k==0)\textbackslash{}n \{\textbackslash{}n sum++;\textbackslash{}n f(k,m/k);\textbackslash{}n \}\textbackslash{}n \textbackslash{}n \}\textbackslash{}n \textbackslash{}n \}\textbackslash{}nOutput: 2\textbackslash{}n\textbackslash{}nInput: int x{[}1000{]}=\{0\};\textbackslash{}nvoid f(int m,int n,int l)\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint i;\textbackslash{}n\textbackslash{}tfor(i=m;i\textless{}=n;i++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tif(n\%i!=0) continue;\textbackslash{}n\textbackslash{}t\textbackslash{}telse\textbackslash{}n\textbackslash{}t\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}tif(n/i==1)\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\textbackslash{}tx{[}l{]}++;\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\textbackslash{}treturn;\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\}\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}telse f(i,n/i,l);\textbackslash{}n\textbackslash{}t\textbackslash{}t\}\textbackslash{}n\textbackslash{}t\}\textbackslash{}t\textbackslash{}n\}\textbackslash{}n\textbackslash{}nint main()\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint a{[}1000{]},s,j,sum;\textbackslash{}n\textbackslash{}tcin\textgreater{}\textgreater{}sum;\textbackslash{}n\textbackslash{}tfor(j=1;j\textless{}=sum;j++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tcin\textgreater{}\textgreater{}a{[}j{]};\textbackslash{}n\textbackslash{}t\textbackslash{}ts=2;\textbackslash{}n\textbackslash{}t f(s,a{[}j{]},j);\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}tfor(j=1;j\textless{}=sum;j++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tcout\textless{}\textless{}x{[}j{]}\textless{}\textless{}endl;\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}treturn 0;\textbackslash{}n\}\textbackslash{}nOutput: 3 $\ldots$} \\  

    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 1/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: create a function that counts the number of prime factors of a given number. The input-output pairs show different implementations of this function, with different variable names and control structures. The output values represent the number of prime factors for the given input number. \newline
    \textbf{Demos}: Input: $\backslash$nint sum(int a,int i)$\backslash$n\text{\{}$\backslash$n$\backslash$tint ret=1;$\backslash$n$\backslash$tfor(;i<=sqrt((float)a);i++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tif(a\%i==0)$\backslash$n$\backslash$t$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$t$\backslash$tret+=sum(a/i,i);$\backslash$n$\backslash$t$\backslash$t\text{\}}$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$treturn ret;$\backslash$n\text{\}}$\backslash$nint main()$\backslash$n\text{\{}$\backslash$n$\backslash$tint t,a,j;$\backslash$n$\backslash$tcin>>t;$\backslash$n$\backslash$t$\backslash$n$\backslash$tfor(j=0;j<t;j++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tcin>>a;$\backslash$n$\backslash$t$\backslash$tcout<<sum(a,2)<<endl;$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$treturn 0;$\backslash$n\text{\}}$\backslash$nOutput: 2$\backslash$n$\backslash$nInput: int sum=0;$\backslash$nint main()$\backslash$n\text{\{}$\backslash$n$\backslash$tvoid, $\ldots$} \\                              
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    % \multirowcell{2}[-0.0ex][l]{Expert \\ 2/8}
    % & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: write a function or a set of functions that would count the number of prime factors in a given number and output the result. Each input-output pair provided a different number for the function to calculate. \newline
    % \textbf{Demos}: Input: int fenjie(int a,int b)$\backslash$n\text{\{}$\backslash$n$\backslash$tint i,sign=0,k=0;$\backslash$n$\backslash$tif(a<b) return 0;$\backslash$n$\backslash$telse if(a==b) return 1;$\backslash$n$\backslash$telse$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tfor(i=2;i<=a-1;i++)$\backslash$n$\backslash$t$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$t$\backslash$tif(a\%i==0)$\backslash$n$\backslash$t$\backslash$t$\backslash$t$\backslash$tsign=1;$\backslash$n$\backslash$t$\backslash$t\text{\}}$\backslash$n$\backslash$t$\backslash$tif(sign!=1) return 1;$\backslash$n$\backslash$t$\backslash$telse $\backslash$n$\backslash$t$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$t$\backslash$tfor(i=b;i<=a;i++)$\backslash$n$\backslash$t$\backslash$t$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$t$\backslash$t$\backslash$tif(a\%i==0)$\backslash$n$\backslash$t$\backslash$t$\backslash$t$\backslash$t$\backslash$tk+=fenjie(a/i,i);$\backslash$n$\backslash$t$\backslash$t$\backslash$t\text{\}}$\backslash$n$\backslash$t$\backslash$t$\backslash$tk+=1;$\backslash$n$\backslash$t$\backslash$t$\backslash$treturn k;$\backslash$n$\backslash$t$\backslash$t\text{\}}$\backslash$n$\backslash$t\text{\}}$\backslash$n\text{\}}$\backslash$n$\backslash$n$\backslash$t$\backslash$nint main()$\backslash$n\text{\{} $\backslash$n$\backslash$tint n,a[100],i,k;$\backslash$n$\backslash$tscanf($\backslash$"\%d$\backslash$",\&n);$\backslash$n$\backslash$n$\backslash$tfor(i=1;i<=n;i++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$n$\backslash$t$\backslash$tscanf($\backslash$"\%d$\backslash$",\&k);$\backslash$n$\backslash$t$\backslash$tprintf($\backslash$"\%d$\backslash$$\backslash$n$\backslash$",fenjie(k,2));$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$treturn 0;$\backslash$n\text{\}}$\backslash$n$\backslash$nOutput: 3$\backslash$n$\backslash$nInput: int fenjie(int n,int min)$\backslash$n\text{\{}$\backslash$nint x=0,i;$\backslash$nif(n==1)$\backslash$nreturn 1;$\backslash$nelse$\backslash$n\text{\{}$\backslash$n$\backslash$tfor(i=min;i<=n;i++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tif(n\%i==0)$\backslash$n$\backslash$t$\backslash$tx=x+fenjie(n/i,i);\text{\}}$\backslash$n\text{\}}$\backslash$nreturn x;\text{\}}$\backslash$nmain()$\backslash$n\text{\{}int shu;$\backslash$n$\backslash$tint number,count=1;$\backslash$n$\backslash$tscanf($\backslash$"\%d$\backslash$",\&number);$\backslash$n$\backslash$twhile(count<number)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tscanf($\backslash$"\%d$\backslash$",&shu);$\backslash$n$\backslash$t$\backslash$tprintf($\backslash$"\%d$\backslash$$\backslash$n$\backslash$",fenjie(shu,2));$\backslash$n$\backslash$tcount++;$\backslash$t\text{\}}$\backslash$n$\backslash$tscanf($\backslash$"\%d$\backslash$",&shu);$\backslash$n$\backslash$tprintf($\backslash$"\%d$\backslash$",fenjie(shu,2));$\backslash$n$\backslash$t$\backslash$t$\backslash$n\text{\}}$\backslash$nOutput: 1, $\ldots$} \\
    % \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    % \multirowcell{2}[-0.0ex][l]{Expert \\ 3/8}
    % & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:  create a program that counts the number of prime factors of a given number. The input-output pairs provided by the friend seem to be testing different cases and inputs to make sure the program is functioning correctly. The output in each case seems to be the correct \newline
    % \textbf{Demos}: Input: $\backslash$nint sum(int a,int i)$\backslash$n\text{\{}$\backslash$n$\backslash$tint ret=1;$\backslash$n$\backslash$tfor(;i<=sqrt((float)a);i++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tif(a\%i==0)$\backslash$n$\backslash$t$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$t$\backslash$tret+=sum(a/i,i);$\backslash$n$\backslash$t$\backslash$t\text{\}}$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$treturn ret;$\backslash$n\text{\}}$\backslash$nint main()$\backslash$n\text{\{}$\backslash$n$\backslash$tint t,a,j;$\backslash$n$\backslash$tcin>>t;$\backslash$n$\backslash$t$\backslash$n$\backslash$tfor(j=0;j<t;j++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tcin>>a;$\backslash$n$\backslash$t$\backslash$tcout<<sum(a,2)<<endl;$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$treturn 0;$\backslash$n\text{\}}$\backslash$nOutput: 2$\backslash$n$\backslash$nInput: int sum=0;$\backslash$nint main()$\backslash$n\text{\{}$\backslash$n$\backslash$tvoid, $\ldots$} \\
    % \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    % \multirowcell{2}[-0.0ex][l]{Expert \\ 4/8}
    % & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:   \newline
    % \textbf{Demos}: Input: int sum=0;$\backslash$nvoid recur(int N,int i)$\backslash$n\text{\{}$\backslash$n if(N==1) sum++;$\backslash$n while(i<=N)$\backslash$n \text{\{}$\backslash$n if(N\%i==0) $\backslash$n$\backslash$t$\backslash$t$\backslash$trecur(N/i,i);$\backslash$n i++;$\backslash$n \text{\}}$\backslash$n return ;$\backslash$n\text{\}}$\backslash$nint main()$\backslash$n\text{\{}$\backslash$n int t=0;$\backslash$n cin>>t;$\backslash$n for(int k = 0; k < t; k++)$\backslash$n \text{\{}$\backslash$n int n=0;$\backslash$n cin>>n;$\backslash$n int i=2,res=1;$\backslash$n for(int i =2; i <=n/2;i++)$\backslash$n \text{\{}$\backslash$n if(n\%i==0)$\backslash$n \text{\{}$\backslash$n sum=0;$\backslash$n recur(n/i,i);$\backslash$n res+=sum;$\backslash$n \text{\}}$\backslash$n \text{\}}$\backslash$n cout<<res<<endl;$\backslash$n \text{\}}$\backslash$n return 0;$\backslash$n\text{\}}$\backslash$n$\backslash$nOutput: 2$\backslash$n$\backslash$nInput: int sum=0;$\backslash$nvoid divide(int n,int a)$\backslash$n\text{\{}$\backslash$n$\backslash$tfor(int i=a;i<=n;i++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tif((n\%i==0))$\backslash$n$\backslash$t$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$t$\backslash$tif(n/i==1)$\backslash$n$\backslash$t$\backslash$t$\backslash$t$\backslash$tsum++;$\backslash$n$\backslash$t$\backslash$t$\backslash$telse$\backslash$n$\backslash$t$\backslash$t$\backslash$t$\backslash$tdivide(n/i,i);$\backslash$n$\backslash$t$\backslash$t\text{\}}$\backslash$n$\backslash$t\text{\}}$\backslash$n\text{\}}$\backslash$nint main()$\backslash$n\text{\{}$\backslash$n$\backslash$tint N=0,n=0,i=0;$\backslash$n$\backslash$tcin>>N;$\backslash$n$\backslash$tfor(i=0;i<N;i++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tcin>>n;$\backslash$n$\backslash$t$\backslash$tdivide(n,2);$\backslash$n$\backslash$t$\backslash$tcout<<sum<<endl;$\backslash$n$\backslash$t$\backslash$tsum=0;$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$treturn 0;$\backslash$n\text{\}}$\backslash$nOutput: 2, $\ldots$} \\
    % \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    % \multirowcell{2}[-0.0ex][l]{Expert \\ 5/8}
    % & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: write a function or a set of functions that would count the number of prime factors in a given number and output the result. Each input-output pair provided a different number for the function to calculate.\newline
    % \textbf{Demos}: Input: int k=0;$\backslash$nint y;$\backslash$nint a(int x,int i);$\backslash$nvoid b(int x,int i);$\backslash$nint main()$\backslash$n\text{\{}$\backslash$n$\backslash$tint n,i,x,z;$\backslash$n$\backslash$tscanf($\backslash$"\%d$\backslash$",\&n);$\backslash$n$\backslash$tfor(i=1;i<=n;i++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tscanf($\backslash$"\%d$\backslash$",\&x);$\backslash$n$\backslash$t$\backslash$ty=x;$\backslash$n$\backslash$t$\backslash$tprintf($\backslash$"\%d$\backslash$$\backslash$n$\backslash$",a(x,2));$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$treturn 0;$\backslash$n\text{\}}$\backslash$nint a(int x,int i)$\backslash$n\text{\{}$\backslash$n$\backslash$tk=0;$\backslash$n$\backslash$tb(x,i);$\backslash$n$\backslash$treturn k;$\backslash$n\text{\}}$\backslash$nvoid b(int x,int i)$\backslash$n\text{\{}$\backslash$n$\backslash$tfor(i=i;i<=x;i++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tif(x\%i==0) b(x/i,i);$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$tif(x==1) k=k+1;$\backslash$n\text{\}}$\backslash$nOutput: 2$\backslash$n$\backslash$nInput: int a;$\backslash$nint fj(int x, int y);$\backslash$nint main()$\backslash$n\text{\{}$\backslash$n$\backslash$tint n;$\backslash$n$\backslash$tcin >> n;$\backslash$n$\backslash$tint i;$\backslash$n$\backslash$tfor (i = 1; i <= n; i++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t cin >> a;$\backslash$n$\backslash$t cout << fj(a, 2) << endl;$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$treturn 0;$\backslash$n\text{\}}$\backslash$nint fj(int x, int y)$\backslash$n\text{\{}$\backslash$n$\backslash$tint xnumber = 1;$\backslash$n$\backslash$tint i;$\backslash$n$\backslash$tint b = sqrt(x);$\backslash$n$\backslash$tif (x == 1) return 0;$\backslash$n$\backslash$telse $\backslash$n$\backslash$t$\backslash$tfor (i = y; i <= b; i++)$\backslash$n$\backslash$t$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$t$\backslash$tif (x \% i == 0) xnumber = xnumber + fj(x / i, i);$\backslash$n$\backslash$t$\backslash$t\text{\}}$\backslash$n$\backslash$t$\backslash$treturn xnumber;$\backslash$n\text{\}}$\backslash$nOutput: 2, $\ldots$} \\
    % \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    % \multirowcell{2}[-0.0ex][l]{Expert \\ 6/8}
    % & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: create a function that counts the number of ways an integer can be expressed as a product of two or more positive integers. The input-output pairs provided test the function with different inputs and expect the number of expressions as the output. Based on these pairs, \newline
    % \textbf{Demos}:  Input: void fun(int m, int i); //????$\backslash$nint num ;$\backslash$nint main()$\backslash$n\text{\{}$\backslash$n$\backslash$tint n, i, a;$\backslash$n$\backslash$tcin>>n;$\backslash$n$\backslash$tfor(i = 0; i < n; i++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tcin>>a;$\backslash$n$\backslash$t$\backslash$tnum = 0;$\backslash$n$\backslash$t$\backslash$tfun(a, 2); //????$\backslash$n$\backslash$t$\backslash$tcout<<num + 1<<endl; //???????a=a???????num??1$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$treturn 0;$\backslash$n\text{\}}$\backslash$nvoid fun(int m, int i)$\backslash$n\text{\{}$\backslash$n$\backslash$tint k = sqrt(m);$\backslash$n$\backslash$tfor(i = i; i <= k; i++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tif(m \% i == 0)$\backslash$n$\backslash$t$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$t num++; $\backslash$n$\backslash$t$\backslash$t$\backslash$tfun(m / i, i); //?????????$\backslash$n$\backslash$t$\backslash$t\text{\}}$\backslash$n$\backslash$t\text{\}}$\backslash$n\text{\}}$\backslash$nOutput: 2$\backslash$n$\backslash$nInput: void count(int, int);$\backslash$nint k;$\backslash$n$\backslash$nint main()$\backslash$n\text{\{}$\backslash$n$\backslash$tint n, i, j, m;$\backslash$n$\backslash$tint num;$\backslash$n$\backslash$tcin >> n;$\backslash$n$\backslash$tfor (i = 0; i < n; i++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tk = 0;$\backslash$n$\backslash$t$\backslash$tcin >> num;$\backslash$n$\backslash$t$\backslash$tm = sqrt(num) + 1;$\backslash$n$\backslash$t$\backslash$tfor (j = 2; j < m; j++)$\backslash$n$\backslash$t$\backslash$t$\backslash$tif (num \% j == 0)$\backslash$n$\backslash$t$\backslash$t$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$t$\backslash$t$\backslash$tk++;$\backslash$n$\backslash$t$\backslash$t$\backslash$t$\backslash$tcount(num / j, j);$\backslash$n$\backslash$t$\backslash$t$\backslash$t\text{\}}$\backslash$n$\backslash$t$\backslash$tcout << k + 1 << endl;$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$treturn 0;$\backslash$n\text{\}}$\backslash$nvoid count(int num, int i)$\backslash$n\text{\{}$\backslash$n$\backslash$tint j;$\backslash$n$\backslash$tint n = sqrt(num);$\backslash$n$\backslash$tfor (j = i; j <= n; j++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tif (num \% j == 0)$\backslash$n$\backslash$t$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$t$\backslash$tk++;$\backslash$n$\backslash$t$\backslash$t$\backslash$tcount((num / j), j);$\backslash$n$\backslash$t$\backslash$t\text{\}}$\backslash$n$\backslash$t\text{\}}$\backslash$n\text{\}}$\backslash$nOutput: 3, $\ldots$} \\
    % \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    % \multirowcell{2}[-0.0ex][l]{Expert \\ 7/8}
    % & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: create a program that counts the number of prime factors of a given number. The input-output pairs provided by the friend seem to be testing different cases and inputs to make sure the program is functioning correctly. The output in each case seems to be the correct \newline
    % \textbf{Demos}: Input: $\backslash$n$\backslash$nint f(int a,int min)$\backslash$n\text{\{} $\backslash$n if(a < min)$\backslash$n \text{\{} $\backslash$n return 0; $\backslash$n \text{\}} $\backslash$n $\backslash$n int r= 1; $\backslash$n for(int i = min;i<a;i++)$\backslash$n \text{\{} $\backslash$n if(a\%i == 0)$\backslash$n \text{\{} $\backslash$n r+= f(a/i,i); $\backslash$n \text{\}} $\backslash$n \text{\}} $\backslash$n $\backslash$n return r; $\backslash$n\text{\}} $\backslash$n$\backslash$nmain()$\backslash$n\text{\{}$\backslash$n int n,a,i,j=0,k,m=0,r=0;$\backslash$n scanf($\backslash$"\%d$\backslash$",\&n);$\backslash$n $\backslash$n for(k=0;k<n;k++)$\backslash$n \text{\{}$\backslash$n scanf($\backslash$"\%d$\backslash$",\&a);$\backslash$n $\backslash$n if(k!=n-1) $\backslash$n printf($\backslash$"\%d$\backslash$$\backslash$n$\backslash$",f(a,2));$\backslash$n else$\backslash$n printf($\backslash$"\%d$\backslash$",f(a,2)); $\backslash$n $\backslash$n $\backslash$n $\backslash$n \text{\}} $\backslash$n $\backslash$n $\backslash$n \text{\}}$\backslash$nOutput: 2$\backslash$n$\backslash$nInput: int f(int a,int min)\text{\{}$\backslash$n$\backslash$tif(a<min)$\backslash$n$\backslash$t$\backslash$treturn 0;$\backslash$n$\backslash$tint sum=1;$\backslash$n$\backslash$tfor(int i=min;i<a;i++)\text{\{}$\backslash$n$\backslash$t$\backslash$tif(a\%i==0)$\backslash$n$\backslash$t$\backslash$t$\backslash$tsum+=f(a/i,i);$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$treturn sum;$\backslash$n\text{\}}$\backslash$nint main()\text{\{}$\backslash$n$\backslash$tint n;$\backslash$n$\backslash$tint a[100];$\backslash$n$\backslash$tscanf($\backslash$"\%d$\backslash$",\&n);$\backslash$n$\backslash$tfor(int i=0;i<n;i++)\text{\{}$\backslash$n$\backslash$t$\backslash$tscanf($\backslash$"\%d$\backslash$",\&a[i]);$\backslash$n$\backslash$t$\backslash$ta[i]=f(a[i],2);$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$tfor(int i=0;i<n;i++)\text{\{}$\backslash$n$\backslash$t$\backslash$tprintf($\backslash$"\%d$\backslash$$\backslash$n$\backslash$",a[i]);$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$treturn 0;$\backslash$n\text{\}}$\backslash$n$\backslash$nOutput: 3, $\ldots$} \\
    % \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    % \multirowcell{2}[-0.0ex][l]{Expert \\ 8/8}
    % & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: create a program that counts the number of prime factors of a given number. The input-output pairs provided by the friend seem to be testing different cases and inputs to make sure the program is functioning correctly. The output in each case seems to be the correct \newline
    % \textbf{Demos}: Input: $\backslash$nint main ()$\backslash$n\text{\{}$\backslash$n$\backslash$tint factor(int n,int x);$\backslash$n$\backslash$tint n;$\backslash$n$\backslash$tint i,m;$\backslash$n$\backslash$tint a[100];$\backslash$n$\backslash$n$\backslash$tscanf($\backslash$"\%d$\backslash$",\&m);$\backslash$n$\backslash$tfor(i=0;i<m;i++)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tscanf($\backslash$"\%d$\backslash$",\&n);$\backslash$n$\backslash$t$\backslash$ta[i]=factor(n,2);$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$tfor(i=0;i<m;i++)$\backslash$n$\backslash$t$\backslash$tprintf($\backslash$"\%d$\backslash$$\backslash$n$\backslash$",a[i]);$\backslash$n$\backslash$treturn 0;$\backslash$n\text{\}}$\backslash$n$\backslash$nint factor(int n,int x)$\backslash$n\text{\{}$\backslash$n$\backslash$tint i,f=0;$\backslash$n$\backslash$n$\backslash$tif(n==1)$\backslash$n f=1;$\backslash$n$\backslash$telse$\backslash$n$\backslash$t$\backslash$tfor(i=x;i<=n;i++)$\backslash$n$\backslash$t$\backslash$t$\backslash$tif(n\%i==0)$\backslash$n$\backslash$t$\backslash$t$\backslash$t$\backslash$tf+=factor(n/i,i);$\backslash$n$\backslash$treturn f;$\backslash$n\text{\}}$\backslash$nOutput: 3$\backslash$n$\backslash$nInput: int main()$\backslash$n\text{\{}$\backslash$n$\backslash$tint nFactor(int n, int border);$\backslash$n$\backslash$tint n;$\backslash$n$\backslash$tcin >> n;$\backslash$n$\backslash$tfor (; n >= 1; n--)$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tint a;$\backslash$n$\backslash$t$\backslash$tcin >> a;$\backslash$n$\backslash$t$\backslash$tcout << nFactor(a, a) << endl;$\backslash$n$\backslash$t\text{\}}$\backslash$n$\backslash$treturn 0;$\backslash$n\text{\}}$\backslash$n$\backslash$nint nFactor(int n, int border)$\backslash$n\text{\{}$\backslash$n$\backslash$tif (n == 1) return 1;$\backslash$n$\backslash$telse$\backslash$n$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$tint i, sum = 0;$\backslash$n$\backslash$t$\backslash$tfor (i = border; i >= 2; i --)$\backslash$n$\backslash$t$\backslash$t\text{\{}$\backslash$n$\backslash$t$\backslash$t$\backslash$tif (n \% i == 0)$\backslash$n$\backslash$t$\backslash$t$\backslash$t$\backslash$tsum += nFactor(n / i, i);$\backslash$n$\backslash$t$\backslash$t\text{\}}$\backslash$n$\backslash$t$\backslash$treturn sum;$\backslash$n$\backslash$t\text{\}}$\backslash$n\text{\}}$\backslash$n$\backslash$nOutput: 2, $\ldots$} \\

    \bottomrule
    \end{tabular}
}

\label{tab:appendix_ex_code_x_glue_information_retreival}
\vspace{-0.175in}
\end{table}

==> tables/rebuttal/fianl_prompts/superni/task835_mathdataset_answer_generation.tex <==
% \setstcolor{red}
\begin{table}[t!]
\footnotesize
\centering
\caption{\small \textbf{\rebuttal{The prompts for each expert found by MoP in the mathdataset\_answer\_generation task of the Super-Natural Instructions benchmark~\citep{wang2022super}.}}}
\resizebox{1.00\textwidth}{!}{
    \renewcommand{\arraystretch}{0.95}
    \begin{tabular}{ll}
    \toprule
    
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task}: mathdataset\_answer\_generation} \\
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task Summary}: Answering multiple choices mathematical problem described with an open vocabulary.} \\
    
    \midrule
    {} & \multicolumn{1}{c}{\textbf{Prompts}} \\
    
    \midrule
    \midrule
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 1/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: create various input-output pairs, so the outputs may not necessarily make sense in the context of the input. The instruction was likely for a math or programming problem involving solving equations or calculating probabilities. \newline
    \textbf{Demos}: Input: Convert 0.3324348 nanoseconds to seconds.$\backslash$nOutput: 0.0000000003324348$\backslash$n$\backslash$nInput: Convert 0.3324348 nanoseconds to seconds.$\backslash$nOutput: 0.0000000003324348$\backslash$n$\backslash$nInput: Convert 0.3324348 nanoseconds to seconds.$\backslash$nOutput: 0.0000000003324348$\backslash$n$\backslash$nInput: Convert 0.3324348 nanoseconds to seconds.$\backslash$nOutput: 0.0000000003324348, $\ldots$} \\                              
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 2/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: perform a calculation or solve an equation, and the output varies depending on the specific inputs given. \newline
    \textbf{Demos}: Input: Let p(s) be the first derivative of s**3/3 + s**2 + 3. Let v be p(-2). What is the units digit of 11/(-1)*(v + -1)?$\backslash$nOutput: 1$\backslash$n$\backslash$nInput: Let s(g) = g**2 - 12*g + 3. Let i be s(12). Solve 1 = 2*p - 4*q + i, 0 = 4*q - 12 for p.$\backslash$nOutput: 5$\backslash$n$\backslash$nInput: Suppose a - f + 0*f + 5 = 0, 5*f = -4*a + 25. Solve a*r + 2*r = 0 for r.$\backslash$nOutput: 0$\backslash$n$\backslash$nInput: Suppose q + 3*d + 13 = -0*q, 2*q + d = -6. Let i = q + 10. Calculate the highest common divisor of 9 and i.$\backslash$nOutput: 9, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 3/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:  create various input-output pairs, so the outputs may not necessarily make sense in the context of the input. The instruction was likely for a math or programming problem involving solving equations or calculating probabilities. \newline
    \textbf{Demos}: Input: Two letters picked without replacement from {x: 3, b: 2}. Give prob of picking 2 x.$\backslash$nOutput: 3/10$\backslash$n$\backslash$nInput: Four letters picked without replacement from {w: 2, k: 1, o: 1, a: 2, b: 2}. What is prob of picking 1 k, 2 a, and 1 b?$\backslash$nOutput: 1/35$\backslash$n$\backslash$nInput: Four letters picked without replacement from {s: 1, u: 1, v: 1, o: 2, f: 2, j: 1}. Give prob of picking 1 v, 1 u, 1 j, and 1 s.$\backslash$nOutput: 1/70, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 4/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:  solve the given equations and provide the value of the specified variable in each output. The input-output pairs provided the results for different sets of equations and variables. In the first pair, the instruction asked to solve for s using the given equations and the value \newline
    \textbf{Demos}: Input: How many micrometers are there in 15/4 of a millimeter?$\backslash$nOutput: 3750$\backslash$n$\backslash$nInput: What is eighteen fifths of a litre in millilitres?$\backslash$nOutput: 3600$\backslash$n$\backslash$nInput: How many millimeters are there in 11/10 of a centimeter?$\backslash$nOutput: 11$\backslash$n$\backslash$nInput: What is twenty-one eighths of a centimeter in micrometers?$\backslash$nOutput: 26250, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 5/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: perform a calculation or solve an equation, and the output varies depending on the specific inputs given. \newline
    \textbf{Demos}: Input: What is the remainder when 46 is divided by (5*-5)/(19 - 20)?$\backslash$nOutput: 21$\backslash$n$\backslash$nInput: Calculate (492/(-287))/((-30)/(-21)).$\backslash$nOutput: -6/5$\backslash$n$\backslash$nInput: What is the value of 32/16*(-6)/(-22)?$\backslash$nOutput: 6/11$\backslash$n$\backslash$nInput: What is the tens digit of (2 - (-12)/(-8))/(2/332)?$\backslash$nOutput: 8$\backslash$n$\backslash$nInput: Calculate ((-12)/(-50))/((-20)/50).$\backslash$nOutput: -3/5, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 6/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:  create various input-output pairs, so the outputs may not necessarily make sense in the context of the input. The instruction was likely for a math or programming problem involving solving equations or calculating probabilities. \newline
    \textbf{Demos}: Input: Suppose -2*c + 4*j - 30 = 2*j, -5*c = -2*j + 78. Let w be 3/12 + (-12)/c. Solve 2*r = -w - 3 for r.$\backslash$nOutput: -2$\backslash$n$\backslash$nInput: Suppose 3*y = -v + 6, -v + 4 = v - 2*y. Suppose 0 = -3*a - 2*c + 1, -4*c + 1 = -3*a - 8*c. Suppose h = 3 + a. Calculate the remainder when h is divided by v.$\backslash$nOutput: 1,, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 7/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:  solve the given equations and provide the value of the specified variable in each output. The input-output pairs provided the results for different sets of equations and variables. In the first pair, the instruction asked to solve for s using the given equations and the value \newline
    \textbf{Demos}: What is 7/4 of a year in months?$\backslash$nOutput: 21$\backslash$n$\backslash$nInput: What is five quarters of a century in months?$\backslash$nOutput: 1500$\backslash$n$\backslash$nInput: How many centuries are there in 78115.17 years?$\backslash$nOutput: 781.1517, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 8/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: create various input-output pairs, so the outputs may not necessarily make sense in the context of the input. The instruction was likely for a math or programming problem involving solving equations or calculating probabilities. \newline
    \textbf{Demos}: Input: Two letters picked without replacement from gga. Give prob of sequence ga.$\backslash$nOutput: 1/3$\backslash$n$\backslash$nInput: Two letters picked without replacement from naioiaaiaaaia. Give prob of picking 1 n and 1 i.$\backslash$nOutput: 2/39$\backslash$n$\backslash$nInput: Two letters picked without replacement from hppfa. Give prob of sequence hf.$\backslash$nOutput: 1/20, $\ldots$} \\

    \bottomrule
    \end{tabular}
}
\label{tab:appendix_ex_mathdataset_answer_generation}
% \vspace{-0.175in}
\end{table}

==> tables/rebuttal/fianl_prompts/superni/task921_code_x_glue_information_retreival.tex <==
% \setstcolor{red}
\begin{table}[t!]
\footnotesize
\centering
\caption{\small \textbf{\rebuttal{The prompts for each expert found by MoP in the code\_x\_glue\_information\_retreival task of the Super-Natural Instructions benchmark~\citep{wang2022super}.}}}
\resizebox{1.00\textwidth}{!}{
    \renewcommand{\arraystretch}{0.95}
    \begin{tabular}{ll}
    \toprule
    
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task}: code\_x\_glue\_information\_retreival} \\
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task Summary}: Given a code, calculate the number of "for loops" in the cpp program.} \\
    \midrule
    {} & \multicolumn{1}{c}{\textbf{Prompts}} \\
    
    \midrule
    \midrule

    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 1/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: create a function that counts the number of prime factors of a given number. The input-output pairs show different implementations of this function, with different variable names and control structures. The output values represent the number of prime factors for the given input number. \newline
    \textbf{Demos}: Input: void f(int i,int m);\textbackslash{}nint sum;\textbackslash{}nint main()\textbackslash{}n\{\textbackslash{}n int n,i,m,k;\textbackslash{}n scanf(\textbackslash{}"\%d\textbackslash{}",\&n);\textbackslash{}n for(i=0;i\textless{}n;i++)\textbackslash{}n \{ sum=1;\textbackslash{}n scanf(\textbackslash{}"\%d\textbackslash{}",\&m);\textbackslash{}n f(2,m);\textbackslash{}n printf(\textbackslash{}"\%d\textbackslash{}\textbackslash{}n\textbackslash{}",sum);\textbackslash{}n \textbackslash{}n \}\textbackslash{}n\}\textbackslash{}n void f(int i ,int m)\textbackslash{}n \{\textbackslash{}n int k,s;\textbackslash{}n s=(int)sqrt(m);\textbackslash{}n for(k=i;k\textless{}=s;k++)\textbackslash{}n \{\textbackslash{}n if(m\%k==0)\textbackslash{}n \{\textbackslash{}n sum++;\textbackslash{}n f(k,m/k);\textbackslash{}n \}\textbackslash{}n \textbackslash{}n \}\textbackslash{}n \textbackslash{}n \}\textbackslash{}nOutput: 2\newline\textbackslash{}n\textbackslash{}nInput: int x{[}1000{]}=\{0\};\textbackslash{}nvoid f(int m,int n,int l)\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint i;\textbackslash{}n\textbackslash{}tfor(i=m;i\textless{}=n;i++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tif(n\%i!=0) continue;\textbackslash{}n, $\ldots$} \\                              
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 2/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: write a function or a set of functions that would count the number of prime factors in a given number and output the result. Each input-output pair provided a different number for the function to calculate. \newline
    \textbf{Demos}: Input: int fenjie(int a,int b)\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint i,sign=0,k=0;\textbackslash{}n\textbackslash{}tif(a\textless{}b) return 0;\textbackslash{}n\textbackslash{}telse if(a==b) return 1;\textbackslash{}n\textbackslash{}telse\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tfor(i=2;i\textless{}=a-1;i++)\textbackslash{}n\textbackslash{}t\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}tif(a\%i==0)\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\textbackslash{}tsign=1;\textbackslash{}n\textbackslash{}t\textbackslash{}t\}\textbackslash{}n\textbackslash{}t\textbackslash{}tif(sign!=1) return 1;\textbackslash{}n\textbackslash{}t\textbackslash{}telse \textbackslash{}n\textbackslash{}t\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}tfor(i=b;i\textless{}=a;i++)\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\textbackslash{}tif(a\%i==0)\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\textbackslash{}t\textbackslash{}tk+=fenjie(a/i,i)\newline \textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\}\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}tk+=1;\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}treturn k;\textbackslash{}n\textbackslash{}t\textbackslash{}t\}\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\}\textbackslash{}n\textbackslash{}n\textbackslash{}t\textbackslash{}nint main()\textbackslash{}n\{ \textbackslash{}n\textbackslash{}tint n,a{[}100{]},i,k;\textbackslash{}n\textbackslash{}tscanf(\textbackslash{}"\%d\textbackslash{}",\&n);\textbackslash{}n\textbackslash{}n\textbackslash{}tfor(i=1;i\textless{}=n;i++)\textbackslash{}n\textbackslash{}t \newline \{\textbackslash{}n\textbackslash{}n\textbackslash{}t\textbackslash{}tscanf(\textbackslash{}"\%d\textbackslash{}",\&k);\textbackslash{}n\textbackslash{}t\textbackslash{}tprintf(\textbackslash{}"\%d\textbackslash{}\textbackslash{}n\textbackslash{}",fenjie(k,2));\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}treturn 0;\textbackslash{}n\}\textbackslash{}n\textbackslash{}nOutput: 3\newline \textbackslash{}n\textbackslash{}n 
    Input: int fenjie(int n,int min)\textbackslash{}n\{\textbackslash{}nint x=0,i;\textbackslash{}nif(n==1)\textbackslash{}nreturn 1;\textbackslash{}nelse\textbackslash{}n\{\textbackslash{}n\textbackslash{}tfor(i=min;i\textless{}=n;i++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tif(n\%i==0)\textbackslash{}n\textbackslash{}t\textbackslash{}tx=x+fenjie(n/i,i);\}\textbackslash{}n\}\textbackslash{}nreturn x;\}\textbackslash{}nmain()\textbackslash{}n\{int shu;\textbackslash{}n\textbackslash{}tint number,count=1;\textbackslash{}n\textbackslash{}tscanf(\textbackslash{}"\%d\textbackslash{}",\&number);\textbackslash{}n, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 3/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:  create a program that counts the number of prime factors of a given number. The input-output pairs provided by the friend seem to be testing different cases and inputs to make sure the program is functioning correctly. The output in each case seems to be the correct \newline
    \textbf{Demos}: Input: \textbackslash{}nint sum(int a,int i)\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint ret=1;\textbackslash{}n\textbackslash{}tfor(;i\textless{}=sqrt((float)a);i++)\textbackslash{}n\textbackslash{}t \newline \{\textbackslash{}n\textbackslash{}t\textbackslash{}tif(a\%i==0)\textbackslash{}n\textbackslash{}t\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}tret+=sum(a/i,i);\textbackslash{}n\textbackslash{}t\textbackslash{}t\}\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}treturn ret;\textbackslash{}n\}\textbackslash{}nint main()\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint t,a,j;\textbackslash{}n\textbackslash{}tcin\textgreater{}\textgreater{}t;\textbackslash{}n\textbackslash{}t\textbackslash{}n\textbackslash{}tfor(j=0;j\textless{}t;j++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tcin\textgreater{}\textgreater{}a;\textbackslash{}n\textbackslash{}t\textbackslash{}tcout\newline \textless{}\textless{}sum(a,2)\textless{}\textless{}endl;\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}treturn 0;\textbackslash{}n\}\textbackslash{}nOutput: 2\newline\textbackslash{}n\textbackslash{}nInput: int sum=0;\textbackslash{}nint main()\textbackslash{}n\{\textbackslash{}n\textbackslash{}tvoid yinshu(int,int), $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 4/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}:   \newline
    \textbf{Demos}: Input: int sum=0;\textbackslash{}nvoid recur(int N,int i)\textbackslash{}n\{\textbackslash{}n if(N==1) sum++;\textbackslash{}n while(i\textless{}=N)\textbackslash{}n \{\textbackslash{}n if(N\%i==0) \textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}trecur(N/i,i);\textbackslash{}n i++;\textbackslash{}n \}\textbackslash{}n return ;\textbackslash{}n\}\textbackslash{}nint main()\textbackslash{}n\{\textbackslash{}n int t=0;\textbackslash{}n cin\textgreater{}\textgreater{}t;\textbackslash{}n for(int k = 0; k \textless t; k++)\textbackslash{}n \{\textbackslash{}n int n=0;\textbackslash{}n cin\textgreater{}\textgreater{}n;\textbackslash{}n int i=2,res=1;\textbackslash{}n for(int i =2; i \textless{}=n/2;i++)\textbackslash{}n \{\textbackslash{}n if(n\%i==0)\textbackslash{}n \{\textbackslash{}n sum=0;\textbackslash{}n recur(n/i,i);\textbackslash{}n res+=sum;\textbackslash{}n \}\textbackslash{}n \}\textbackslash{}n cout\textless{}\textless{}res\textless{}\textless{}endl;\textbackslash{}n \}\textbackslash{}n return 0;\textbackslash{}n\}\textbackslash{}n\textbackslash{}nOutput: 2\textbackslash{}n\textbackslash{}nInput: int sum=0;\textbackslash{}nvoid divide(int n,int a)\textbackslash{}n\{\textbackslash{}n\textbackslash{}tfor(int i=a;i\textless{}=n;i++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tif((n\%i==0))\textbackslash{}n\textbackslash{}t\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}tif(n/i==1)\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\textbackslash{}tsum++;\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}telse\newline \textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\textbackslash{}tdivide(n/i,i);\textbackslash{}n\textbackslash{}t\textbackslash{}t\}\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\}\textbackslash{}nint main()\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint N=0,n=0,i=0;\textbackslash{}n\textbackslash{}tcin\textgreater{}\textgreater{}N;\textbackslash{}n\newline \textbackslash{}tfor(i=0;i\textless{}N;i++) 
    \textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tcin\textgreater{}\textgreater{}n;\textbackslash{}n\textbackslash{}t\textbackslash{}tdivide(n,2);\textbackslash{}n\textbackslash{}t\textbackslash{}tcout\textless{}\textless{}sum\textless{}\textless{}endl;\newline\textbackslash{}n\textbackslash{}t\textbackslash{}tsum=0;\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}treturn 0;\textbackslash{}n\}\textbackslash{}nOutput: 2, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 5/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: write a function or a set of functions that would count the number of prime factors in a given number and output the result. Each input-output pair provided a different number for the function to calculate.\newline
    \textbf{Demos}: Input: int k=0;\textbackslash{}nint y;\textbackslash{}nint a(int x,int i);\textbackslash{}nvoid b(int x,int i);\textbackslash{}nint main()\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint n,i,x,z;\textbackslash{}n\textbackslash{}tscanf(\textbackslash{}"\%d\textbackslash{}",\&n);\textbackslash{}n\textbackslash{}tfor(i=1;i\textless{}=n;i++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tscanf(\textbackslash{}"\%d\textbackslash{}",\&x);\textbackslash{}n\textbackslash{}t\textbackslash{}ty=x;\newline \textbackslash{}n\textbackslash{}t\textbackslash{}t printf(\textbackslash{}"\%d\textbackslash{}\textbackslash{}n\textbackslash{}",a(x,2));\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}treturn 0;\textbackslash{}n\}\textbackslash{}nint a(int x,int i)\textbackslash{}n\{\textbackslash{}n\textbackslash{}tk=0;\textbackslash{}n\textbackslash{}tb(x,i);\textbackslash{}n\textbackslash{}treturn k;\textbackslash{}n\}\textbackslash{}nvoid b(int x,int i)\textbackslash{}n\{\textbackslash{}n\textbackslash{}tfor(i=i;i\textless{}=x;i++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}t \newline if(x\%i==0) b(x/i,i);\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}tif(x==1) k=k+1;\textbackslash{}n\}\textbackslash{}nOutput: 2\textbackslash{}n\textbackslash{}nInput: int a;\textbackslash{}nint fj(int x, int y);\textbackslash{}nint main()\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint n;\textbackslash{}n\textbackslash{}tcin \textgreater{}\textgreater n;\textbackslash{}n\textbackslash{}tint i;\textbackslash{}n\textbackslash{}tfor (i = 1; i \textless{}= n; i++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t cin \textgreater{}\textgreater a;\textbackslash{}n\textbackslash{}t cout \textless{}\textless fj(a, 2) \textless{}\textless endl;\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}treturn 0;\textbackslash{}n\}\textbackslash{}nint fj(int x, int y)\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint xnumber = 1;\textbackslash{}n\textbackslash{}tint i;\textbackslash{}n\textbackslash{}tint b = sqrt(x);\textbackslash{}n\textbackslash{}tif (x == 1) return 0;\textbackslash{}n\textbackslash{}telse \textbackslash{}n\textbackslash{}t\textbackslash{}tfor (i = y; i \textless{}= b; i++)\textbackslash{}n\textbackslash{}t\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}tif (x \% i == 0) xnumber = xnumber + fj(x / i, i);\textbackslash{}n\textbackslash{}t\textbackslash{}t\}\textbackslash{}n\textbackslash{}t\textbackslash{}treturn xnumber;\textbackslash{}n\}\textbackslash{}nOutput: 2, $\ldots$} \\
    % \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    

    \bottomrule
    \end{tabular}
}

\label{tab:appendix_ex_code_x_glue_information_retreival}
% \vspace{-0.175in}
\end{table}

==> tables/rebuttal/fianl_prompts/superni/task921_code_x_glue_information_retreival_2.tex <==
% \setstcolor{red}
\begin{table}[t!]
\footnotesize
\centering
\caption{\small \textbf{\rebuttal{(The extension of~\Cref{tab:appendix_ex_code_x_glue_information_retreival}) The prompts for each expert found by MoP in the code\_x\_glue\_information\_retreival task of the Super-Natural Instructions benchmark~\citep{wang2022super}.}}}
\resizebox{1.00\textwidth}{!}{
    \renewcommand{\arraystretch}{0.95}
    \begin{tabular}{ll}
    \toprule
    
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task}: code\_x\_glue\_information\_retreival} \\
    \multicolumn{2}{p{1.0\textwidth}}{\textbf{Task Summary}: Given a code, calculate the number of "for loops" in the cpp program.} \\
    \midrule
    {} & \multicolumn{1}{c}{\textbf{Prompts}} \\
    
    \midrule
    \midrule

    \multirowcell{2}[-0.0ex][l]{Expert \\ 6/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: create a function that counts the number of ways an integer can be expressed as a product of two or more positive integers. The input-output pairs provided test the function with different inputs and expect the number of expressions as the output. Based on these pairs, \newline
    \textbf{Demos}:  Input: void fun(int m, int i); //????\textbackslash{}nint num ;\textbackslash{}nint main()\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint n, i, a;\textbackslash{}n\textbackslash{}tcin\textgreater{}\textgreater{}n;\textbackslash{}n\textbackslash{}tfor(i = 0; i \textless n; i++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tcin\textgreater{}\textgreater{}a;\textbackslash{}n\textbackslash{}t\textbackslash{}tnum = 0;\textbackslash{}n\textbackslash{}t\textbackslash{}tfun(a, 2); //????\textbackslash{}n\textbackslash{}t\textbackslash{}tcout\textless{}\textless{}num + 1\textless{}\textless{}endl; //???????a=a???????num??1\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}treturn 0;\textbackslash{}n\}\textbackslash{}nvoid fun(int m, int i)\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint k = sqrt(m);\textbackslash{}n\textbackslash{}tfor(i = i; i \textless{}= k; i++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tif(m \% i == 0)\textbackslash{}n\textbackslash{}t\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}t num++; \textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}tfun(m / i, i); //?????????\textbackslash{}n\textbackslash{}t\textbackslash{}t\}\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\}\textbackslash{}nOutput: 2\textbackslash{}n\textbackslash{}nInput: void count(int, int);\textbackslash{}nint k;\textbackslash{}n\textbackslash{}nint main()\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint n, i, j, m;\textbackslash{}n\textbackslash{}tint num;\textbackslash{}n\textbackslash{}tcin \textgreater{}\textgreater n;\textbackslash{}n\textbackslash{}tfor (i = 0; i \textless n; i++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tk = 0;\textbackslash{}n\textbackslash{}t\textbackslash{}tcin \textgreater{}\textgreater num;\textbackslash{}n\textbackslash{}t\textbackslash{}tm = sqrt(num) + 1;\textbackslash{}n\textbackslash{}t\textbackslash{}tfor (j = 2; j \textless m; j++)\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}tif (num \% j == 0)\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\textbackslash{}tk++;\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\textbackslash{}tcount(num / j, j);\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\}\textbackslash{}n\textbackslash{}t\textbackslash{}tcout \textless{}\textless k + 1 \textless{}\textless endl;\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}treturn 0;\textbackslash{}n\}\textbackslash{}nvoid count(int num, int i)\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint j;\textbackslash{}n\textbackslash{}tint n = sqrt(num);\textbackslash{}n\textbackslash{}tfor (j = i; j \textless{}= n; j++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tif (num \% j == 0)\textbackslash{}n\textbackslash{}t\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}tk++;\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}tcount((num / j), j);\textbackslash{}n\textbackslash{}t\textbackslash{}t\}\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\}\textbackslash{}nOutput: 3, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 7/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: create a program that counts the number of prime factors of a given number. The input-output pairs provided by the friend seem to be testing different cases and inputs to make sure the program is functioning correctly. The output in each case seems to be the correct \newline
    \textbf{Demos}: Input: int f(int a,int min)\{\textbackslash{}n\textbackslash{}tif(a\textless{}min)\textbackslash{}n\textbackslash{}t\textbackslash{}treturn 0;\textbackslash{}n\textbackslash{}tint sum=1;\textbackslash{}n\textbackslash{}tfor(int i=min;i\textless{}a;i++)\{\textbackslash{}n\textbackslash{}t\textbackslash{}tif(a\%i==0)\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}tsum+=f(a/i,i);\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}treturn sum;\textbackslash{}n\}\textbackslash{}nint main()\{\textbackslash{}n\textbackslash{}tint n;\textbackslash{}n\textbackslash{}tint a{[}100{]};\textbackslash{}n\textbackslash{}tscanf(\textbackslash{}"\%d\textbackslash{}",\&n);\textbackslash{}n\textbackslash{}tfor(int i=0;i\textless{}n;i++)\{\textbackslash{}n\textbackslash{}t\textbackslash{}tscanf(\textbackslash{}"\%d\textbackslash{}",\&a{[}i{]});\textbackslash{}n\textbackslash{}t\textbackslash{}ta{[}i{]}=f(a{[}i{]},2);\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}tfor(int i=0;i\textless{}n;i++)\{\textbackslash{}n\textbackslash{}t\textbackslash{}tprintf(\textbackslash{}"\%d\textbackslash{}\textbackslash{}n\textbackslash{}",a{[}i{]});\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}treturn 0;\textbackslash{}n\}\textbackslash{}n\textbackslash{}nOutput: 3\textbackslash{}n\textbackslash{}nInput: \textbackslash{}nint f(int a,int min)\textbackslash{}n\{ \textbackslash{}nif(a \textless min)\textbackslash{}n\{ \textbackslash{}nreturn 0; \textbackslash{}n\} \textbackslash{}nint result = 1; \textbackslash{}nfor(int i = min;i\textless{}a;i++)\textbackslash{}n\{ \textbackslash{}nif(a \% i == 0)\textbackslash{}n\{ \textbackslash{}nresult += f(a/i,i); \textbackslash{}n\} \textbackslash{}n\} \textbackslash{}nreturn result; \textbackslash{}n\} \textbackslash{}n\textbackslash{}nmain()\textbackslash{}n\{\textbackslash{}n int n;\textbackslash{}n scanf(\textbackslash{}"\%d\textbackslash{}",\&n);\textbackslash{}n int i;\textbackslash{}n int a;\textbackslash{}n int b;\textbackslash{}n for(i=0;i\textless{}n;i++)\textbackslash{}n \{\textbackslash{}n scanf(\textbackslash{}"\%d\textbackslash{}",\&a);\textbackslash{}n int min=2;\textbackslash{}n b=f(a,2);\textbackslash{}n printf(\textbackslash{}"\%d\textbackslash{}",b);\textbackslash{}n printf(\textbackslash{}"\textbackslash{}\textbackslash{}n\textbackslash{}"); \textbackslash{}n \}\textbackslash{}n \}\textbackslash{}n\textbackslash{}nOutput: 2, $\ldots$} \\
    \noalign{\vskip 0.5ex}\cdashline{0-1}\noalign{\vskip 0.75ex}
    
    \multirowcell{2}[-0.0ex][l]{Expert \\ 8/8}
    & \multicolumn{1}{p{0.9\textwidth}}{\textbf{Instruction}: create a program that counts the number of prime factors of a given number. The input-output pairs provided by the friend seem to be testing different cases and inputs to make sure the program is functioning correctly. The output in each case seems to be the correct \newline
    \textbf{Demos}: Input: \textbackslash{}nint main ()\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint factor(int n,int x);\textbackslash{}n\textbackslash{}tint n;\textbackslash{}n\textbackslash{}tint i,m;\textbackslash{}n\textbackslash{}tint a{[}100{]};\textbackslash{}n\textbackslash{}n\textbackslash{}tscanf(\textbackslash{}"\%d\textbackslash{}",\&m);\textbackslash{}n\textbackslash{}tfor(i=0;i\textless{}m;i++)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tscanf(\textbackslash{}"\%d\textbackslash{}",\&n);\newline \textbackslash{}n\textbackslash{}t\textbackslash{}ta{[}i{]}=factor(n,2);\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}tfor(i=0;i\textless{}m;i++)\textbackslash{}n\textbackslash{}t\textbackslash{}tprintf(\textbackslash{}"\%d\textbackslash{}\textbackslash{}n\textbackslash{}",a{[}i{]});\textbackslash{}n\textbackslash{}treturn 0;\textbackslash{}n\}\textbackslash{}n\textbackslash{}nint factor(int n,int x)\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint i,f=0;\textbackslash{}n\textbackslash{}n\textbackslash{}tif(n==1)\textbackslash{}n f=1;\textbackslash{}n\textbackslash{}telse\textbackslash{}n\textbackslash{}t\textbackslash{}tfor(i=x;i\textless{}=n;i++)\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}tif(n\%i==0)\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\textbackslash{}tf+=factor(n/i,i);\textbackslash{}n\textbackslash{}treturn f;\textbackslash{}n\}\textbackslash{}nOutput: 3\textbackslash{}n\textbackslash{}nInput: int main()\textbackslash{}n\{\textbackslash{}n\textbackslash{}tint nFactor(int n, int border);\textbackslash{}n\textbackslash{}tint n;\textbackslash{}n\textbackslash{}tcin \textgreater{}\textgreater n;\textbackslash{}n\textbackslash{}tfor (; n \textgreater{}= 1; n--)\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tint a;\textbackslash{}n\textbackslash{}t\textbackslash{}tcin \textgreater{}\textgreater a;\textbackslash{}n\textbackslash{}t\textbackslash{}tcout \textless{}\textless nFactor(a, a) \textless{}\textless endl;\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\textbackslash{}treturn 0;\textbackslash{}n\}\textbackslash{}n\textbackslash{}nint nFactor(int n, int border)\textbackslash{}n\{\textbackslash{}n\textbackslash{}tif (n == 1) return 1;\textbackslash{}n\textbackslash{}telse\textbackslash{}n\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}tint i, sum = 0;\textbackslash{}n\textbackslash{}t\textbackslash{}tfor (i = border; i \textgreater{}= 2; i --)\textbackslash{}n\textbackslash{}t\textbackslash{}t\{\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}tif (n \% i == 0)\textbackslash{}n\textbackslash{}t\textbackslash{}t\textbackslash{}t\textbackslash{}tsum += nFactor(n / i, i);\textbackslash{}n\textbackslash{}t\textbackslash{}t\}\textbackslash{}n\textbackslash{}t\textbackslash{}treturn sum;\textbackslash{}n\textbackslash{}t\}\textbackslash{}n\}\textbackslash{}n\textbackslash{}nOutput: 2, $\ldots$} \\

    \bottomrule
    \end{tabular}
}

\label{tab:appendix_ex_code_x_glue_information_retreival_2}
% \vspace{-0.175in}
\end{table}

==> tables/rebuttal/fianl_prompts/superni/temp.tex <==
structures. The output values represent the number of prime factors for the given input number.\n\nInput: void f(int i,int m);\nint sum;\nint main()\n{\n int n,i,m,k;\n scanf(\"%d\",&n);\n for(i=0;i<n;i++)\n { sum=1;\n scanf(\"%d\",&m);\n f(2,m);\n printf(\"%d\\n\",sum);\n \n }\n}\n void f(int i ,int m)\n {\n int k,s;\n s=(int)sqrt(m);\n for(k=i;k<=s;k++)\n {\n if(m%k==0)\n {\n sum++;\n f(k,m/k);\n }\n \n }\n \n }\nOutput: 2\n\nInput: int x[1000]={0};\nvoid f(int m,int n,int l)\n{\n\tint i;\n\tfor(i=m;i<=n;i++)\n\t{\n\t\tif(n%i!=0) continue;\n\t\telse\n\t\t{\n\t\t\tif(n/i==1)\n\t\t\t{\n\t\t\t\tx[l]++;\n\t\t\t\treturn;\n\t\t\t}\n\t\t\telse f(i,n/i,l);\n\t\t}\n\t}\t\n}\n\nint main()\n{\n\tint a[1000],s,j,sum;\n\tcin>>sum;\n\tfor(j=1;j<=sum;j++)\n\t{\n\t\tcin>>a[j];\n\t\ts=2;\n\t f(s,a[j],j);\n\t}\n\tfor(j=1;j<=sum;j++)\n\t{\n\t\tcout<<x[j]<<endl;\n\t}\n\treturn 0;\n}\nOutput: 3…

==> tables/rebuttal/non_gpt_embedding_models.tex <==

% \begin{table}[t!]
% \caption{\small \textbf{Effect of different embedding models on the }. The choice of models and algo-
% rithms in MoP is listed in the last row of every group.
% The best performance is achieved with K-Mean-Auto,
% text-embedding-ada, and region-based joint search.}
% \vspace{-0.1in}
% \tiny
% \begin{center}
% \resizebox{0.7\textwidth}{!}{
% \begin{tabular}{lccc}
% \toprule
% Embedding Model  & sentence\_similarity    & word\_in\_context  & auto\_categorization  \\
                           
% \midrule
% \midrule
% GPT2                                   & 39.50 \tiny$\pm$ 3.57 & 56.25 \tiny$\pm$ 3.63 & 33.75 \tiny$\pm$ 3.11 \\ 
% GPT2-Large                                  & 39.00 \tiny$\pm$ 2.55 & 52.75 \tiny$\pm$ 3.11 & 49.50 \tiny$\pm$ 2.69 \\  
% Sentence-T5                                   & 42.50 \tiny$\pm$ 2.96 & 57.50 \tiny$\pm$ 5.89 & 54.50 \tiny$\pm$ 2.06 \\
% GPT-Ada                & \textbf{43.00 \tiny$\pm$ 3.54} & \textbf{59.00 \tiny$\pm$ 5.15} & \textbf{54.25 \tiny$\pm$ 2.49} \\ 
% \bottomrule
% \end{tabular}
% } 	
% \end{center}
% \label{tbl:suppl_non_gpt_ablate}
% \vspace{-0.15in}
% \end{table}


==> tables/rebuttal/superni.tex <==
\begin{table*}[t!]
\tiny
    \caption{\small \sh{Update finished.} \textbf{Experimental results for the Super-Natural Instructions tasks.} We report the ROUGE-L score for each method. We run 3 experiments and provide both the mean and standard deviation values. Due to innate randomness in ChatGPT API, we mark methods to be equivalent when their accuracy gap falls within 1\%. The number of demos is set to $N_{\text{train}}/5$, where $N_{\text{train}}$ is the total number of training demos.}
    \begin{center}

    \resizebox{\linewidth}{!}{
        \begin{tabular}{cllll}
            \toprule
            \multicolumn{2}{c}{\multirow{2}{*}{Task}} & \multicolumn{3}{c}{Method} \\
            & & \multicolumn{1}{c}{APE~\citep{zhou2022large}} & \multicolumn{1}{c}{APE + K-centroids Demos} & \multicolumn{1}{c}{MoP + K-Means-Auto} \\
            
            \midrule
            \midrule
            
            \multirow{8}{*}{\rotatebox[origin=c]{90}{\tiny Code}} 
            
            & conala\_normalize\_lists                 & 47.85\tiny$\pm$1.11          & 49.15\tiny$\pm$0.44          & 48.76\tiny$\pm$0.76          \\
            & conala\_calculate\_mean                  & 27.02\tiny$\pm$3.20          & 29.78\tiny$\pm$3.94          & 29.60\tiny$\pm$3.37          \\
            & conala\_list\_index\_subtraction          & 47.48\tiny$\pm$13.80         & 49.92\tiny$\pm$14.50         & 47.79\tiny$\pm$9.93          \\
            & logic2text\_sentence\_generation         & 38.90\tiny$\pm$2.19          & 86.32\tiny$\pm$1.07          & 97.26\tiny$\pm$1.26          \\
            & conala\_list\_index\_addition            & 46.61\tiny$\pm$5.92          & 49.66\tiny$\pm$3.74          & 49.43\tiny$\pm$17.75         \\
            & conala\_pair\_averages                   & 48.15\tiny$\pm$14.44         & 68.06\tiny$\pm$22.89         & 97.75\tiny$\pm$0.77          \\
            & conala\_pair\_differences                & 10.17\tiny$\pm$5.24          & 26.02\tiny$\pm$14.83         & 67.53\tiny$\pm$15.71          \\
            & code\_x\_glue\_information\_retreival    & 11.51\tiny$\pm$4.18          & 36.67\tiny$\pm$3.09          & 35.00\tiny$\pm$4.08          \\

            \hdashline        
            
            \multirow{13}{*}{\rotatebox[origin=c]{90}{\tiny Mathematics}}
            
            & semeval\_2019\_task10\_closed\_vocabulary  & \multirow{2}{*}{19.33\tiny$\pm$5.86} & \multirow{2}{*}{36.67\tiny$\pm$3.09}     & \multirow{2}{*}{37.00\tiny$\pm$4.32} \\
            & \_mathematical\_answer\_generation & & & \\
            & semeval\_2019\_task10\_open\_vocabulary  & \multirow{2}{*}{20.58\tiny$\pm$3.38} & \multirow{2}{*}{31.67\tiny$\pm$3.30}     & \multirow{2}{*}{32.33\tiny$\pm$2.62} \\
            & \_mathematical\_answer\_generation & & & \\
            & aqua\_multiple\_choice\_answering           & 45.50\tiny$\pm$0.91        &   64.50\tiny$\pm$1.63      & 63.50\tiny$\pm$0.82        \\
            & mathdataset\_classification                 & 32.92\tiny$\pm$20.21       &   78.33\tiny$\pm$4.92      & 95.67\tiny$\pm$2.87        \\
            & mathdataset\_answer\_generation             & 27.99\tiny$\pm$3.61        &   41.81\tiny$\pm$6.15      & 43.67\tiny$\pm$5.48        \\
            & leetcode\_420\_strong\_password\_check      & 1.67\tiny$\pm$2.36         &   9.67\tiny$\pm$4.92       & 26.34\tiny$\pm$6.24        \\
            & mathqa\_gain                                & 15.58\tiny$\pm$4.18        &   25.67\tiny$\pm$3.09      & 29.00\tiny$\pm$2.45        \\
            & mathqa\_general                             & 19.47\tiny$\pm$1.47        &   28.00\tiny$\pm$4.08      & 29.00\tiny$\pm$0.82        \\
            & mathqa\_other                               & 16.61\tiny$\pm$2.58        &   31.00\tiny$\pm$6.98      & 31.00\tiny$\pm$2.16        \\
            & mathqa\_geometry                            & 19.12\tiny$\pm$4.01        &   35.33\tiny$\pm$4.71      & 37.00\tiny$\pm$3.27        \\
            & mathqa\_probability                         & 16.88\tiny$\pm$2.77        &   38.33\tiny$\pm$2.05      & 39.33\tiny$\pm$4.50        \\
            & mathqa\_answer\_selection                   & 19.83\tiny$\pm$1.59        &   27.67\tiny$\pm$3.77      & 30.33\tiny$\pm$7.59        \\
            & mathqa\_correct\_answer\_generation         & 21.57\tiny$\pm$1.74        &   28.56\tiny$\pm$2.62      & 30.76\tiny$\pm$1.55        \\
            
            \bottomrule
            \end{tabular}
        }
    \end{center}
    \label{tbl:superni}
\end{table*}


==> tables/win_rate.tex <==
\begin{table}[t]
    \caption{\small \textbf{Pairwise win rate.}}

    \centering
    \resizebox{1.0\linewidth}{!}{
    \renewcommand{\arraystretch}{0.95}
    \renewcommand{\tabcolsep}{8pt}
    \begin{tabular}{lccccccc}
    
        \toprule
        
        & \multicolumn{7}{c}{\textbf{Instruction Induction}} \\
        
        \cmidrule(l{2pt}r{2pt}){2-8}
        % \cmidrule(l{2pt}r{2pt}){9-15}
        
        \textbf{Method} & \textbf{APE} & \textbf{APE+R} & \textbf{APE+K} & \textbf{IZ} & \textbf{IZ+R} & \textbf{IZ+K} &  \textbf{MoP} \\
        \midrule
        \midrule
    
        \textbf{APE} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{APE+R} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{APE+K} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{IZ} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{IZ+R} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{IZ+K} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{\cellcolor{gray!25}MoP} & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx \\
        
        \bottomrule
    \end{tabular}
    }

    \resizebox{1.0\linewidth}{!}{
    \renewcommand{\arraystretch}{0.95}
    \renewcommand{\tabcolsep}{8pt}
    \begin{tabular}{lccccccc}
    
        \toprule
        
        & \multicolumn{7}{c}{\textbf{Super Natural Instructions}} \\
        
        \cmidrule(l{2pt}r{2pt}){2-8}
        % \cmidrule(l{2pt}r{2pt}){9-15}
        
        \textbf{Method} & \textbf{APE} & \textbf{APE+R} & \textbf{APE+K} & \textbf{IZ} & \textbf{IZ+R} & \textbf{IZ+K} &  \textbf{MoP} \\
        \midrule
        \midrule
    
        \textbf{APE} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{APE+R} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{APE+K} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{IZ} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{IZ+R} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{IZ+K} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{\cellcolor{gray!25}MoP} & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx \\
        
        \bottomrule
    \end{tabular}
    }

    \resizebox{1.0\linewidth}{!}{
    \renewcommand{\arraystretch}{0.95}
    \renewcommand{\tabcolsep}{8pt}
    \begin{tabular}{lccccccc}
    
        \toprule
        
        & \multicolumn{7}{c}{\textbf{BIG-Bench-Hard}} \\
        
        \cmidrule(l{2pt}r{2pt}){2-8}
        % \cmidrule(l{2pt}r{2pt}){9-15}
        
        \textbf{Method} & \textbf{APE} & \textbf{APE+R} & \textbf{APE+K} & \textbf{IZ} & \textbf{IZ+R} & \textbf{IZ+K} &  \textbf{MoP} \\
        \midrule
        \midrule
    
        \textbf{APE} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{APE+R} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{APE+K} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{IZ} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{IZ+R} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{IZ+K} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
        \textbf{\cellcolor{gray!25}MoP} & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx & \cellcolor{gray!25}xx.xx \\
        
        \bottomrule
    \end{tabular}
    }
\label{tab:win_rate}
\end{table}
